DAMIA: Leveraging Domain Adaptation as a Defense against Membership Inference Attacks

Deep Learning (DL) techniques allow ones to train models from a dataset to solve tasks. DL has attracted much interest given its fancy performance and potential market value, while security issues are amongst the most colossal concerns. However, the DL models may be prone to the membership inference attack, where an attacker determines whether a given sample is from the training dataset. Efforts have been made to hinder the attack but unfortunately, they may lead to a major overhead or impaired usability. In this paper, we propose and implement DAMIA, leveraging Domain Adaptation (DA) as a defense aginist membership inference attacks. Our observation is that during the training process, DA obfuscates the dataset to be protected using another related dataset, and derives a model that underlyingly extracts the features from both datasets. Seeing that the model is obfuscated, membership inference fails, while the extracted features provide supports for usability. Extensive experiments have been conducted to validates our intuition. The model trained by DAMIA has a negligible footprint to the usability. Our experiment also excludes factors that may hinder the performance of DAMIA, providing a potential guideline to vendors and researchers to benefit from our solution in a timely manner.

==> TODOs/remaining_problems.tex <==
List of remaining problems:





-------


TODOs:


==> Trashbin/Z-_abandoned_-sec4-evaluation.tex <==
\section{ Evaluation }
\label{sec:evaluation}


\subsection{ Experiments on different domain adaptaion approaches }
\label{sec:experiments_on_different_domain_adaptaion_approaches}

In this section, we conduct experiments to verify whether domain adaption is available to be leveraged as the defense against membership inference. In the experiments, we concentrate on the accuracy of membership inference and test accuracy on the target domain since it acts as the placeholder for our private dataset.
Although there are three types of domain adaptation approaches, whose purposes are all to transfer knowledge from the source to the target by constructing a shared representation, the way that each approach adopt varies and will affect the shared representation. To better achieve our goal and filter out the best approach, we evaluate all the three approaches using datasets shown in \autoref{sub:datasets}.


% 评估 discrepancy-based 方法
\subsubsection{Evaluation on discrepancy-based domain adaptation}

We first evaluate discrepancy-based domain adaptation to investigate the effects of domain adaptation on membership inference. We choose the classical method --- MMD (maximum mean discrepancy) in our experiments.

To eliminate the impact of the architecture of a neural network, we use both AlexNet and ResNet-50 as the backbone of the whole model respectively and train the s for 150 epochs to make sure that they are converged. The experiments are shown in \autoref{tab:exp01_offcie31_alexnet} to \autoref{tab:exp01_mnist_svhn_resnet50}

\begin{table}[H]
    \centering
    \caption{Experiment results of AlexNet on MNSIT and SVHN}
    \label{tab:exp01_mnist_svhn_alexnet}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
        MNIST $\rightarrow$ SVHN & 0.9997      & 0.9949      & 0.212566717 & 0.224953903 & 0.505841667 & 0.503727767 \\ \hline
        SVHN $\rightarrow$ MNIST & 0.978609553 & 0.950138291 & 0.76805     & 0.7702      & 0.561351334 & 0.503108333 \\ \hline

        \end{tabular}%
    }
\end{table}

\begin{table}[H]
    \centering
    \caption{Experiment results of AlexNet on Office 31}
    \label{tab:exp01_offcie31_alexnet}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    Amazon $\rightarrow$ DSLR   & 0.750110963 & 0.686170213 & 0.447236181 & 0.46        & 0.556306721 & 0.528492462 \\ \hline
    Amazon $\rightarrow$ Webcam & 0.813581891 & 0.744680851 & 0.501572327 & 0.459119497 & 0.571273763 & 0.534591195 \\ \hline
    DSLR $\rightarrow$ Amazon   & 1           & 0.91        & 0.407900577 & 0.416666667 & 0.694899497 & 0.510169656 \\ \hline
    DSLR $\rightarrow$ Webcam   & 1           & 0.94        & 0.938679245 & 0.93081761  & 0.663467337 & 0.522012579 \\ \hline
    Webcam $\rightarrow$ Amazon & 1           & 0.981132075 & 0.375055482 & 0.372340426 & 0.619496855 & 0.514514926 \\ \hline
    Webcam $\rightarrow$ DSLR   & 0.98427673  & 0.93081761  & 0.929648241 & 0.91        & 0.639937107 & 0.544296482 \\ \hline
    \end{tabular}%
    } 
\end{table}


\begin{table}[H]
    \centering
    \caption{Experiment results of RenNet-50 on MNSIT and SVHN}
    \label{tab:exp01_mnist_svhn_resnet50}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
        MNIST $\rightarrow$ SVHN & 0.9775      & 0.9751      & 0.219173594 & 0.227566073 & \textbf{0.502416667} & 0.511505038 \\ \hline
        SVHN $\rightarrow$ MNIST & 0.933822024 & 0.915527044 & 0.778966667 & 0.7844      & \textbf{0.522691311} & 0.500133333 \\ \hline
        \end{tabular}%
    }
\end{table}

\begin{table}[H]
    \centering
    \caption{Experiment results of ResNet-50 on Office 31}
    \label{tab:exp01_offcie31_resnet50}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    Amazon $\rightarrow$ DSLR   & 0.817132712 & 0.771276596 & 0.733668342 & 0.68        & \textbf{0.535641603} & \textbf{0.542964824} \\ \hline
    Amazon $\rightarrow$ Webcam & 0.865068797 & 0.794326241 & 0.721698113 & 0.761006289 & \textbf{0.549949949} & \textbf{0.517295597} \\ \hline
    DSLR $\rightarrow$ Amazon   & 1           & 0.97        & 0.625832224 & 0.675531915 & \textbf{0.64459799 } & \textbf{0.507515983} \\ \hline
    DSLR $\rightarrow$ Webcam   & 1           & 0.97        & 0.962264151 & 0.981132075 & \textbf{0.646055276} & \textbf{0.504716981} \\ \hline
    Webcam $\rightarrow$ Amazon & 1           & 0.974842767 & 0.628051487 & 0.663120567 & \textbf{0.625786164} & \textbf{0.501553484} \\ \hline
    Webcam $\rightarrow$ DSLR   & 0.987421384 & 0.974842767 & 0.992462312 & 0.99        & \textbf{0.627358491} & \textbf{0.551909548} \\ \hline
    \end{tabular}%
    }
\end{table}


% 实验结果和简单的观察
% 1. mia acc on target 小于 source
% 2. test acc 和 training acc 之间的差异 与 source 和 target 之间的差异存在联系
% 3. 任务困难度无关，在结果上表现类似 (似乎不是很有必要？)
As shown in the tables, compared to the source training sets, models have lower membership inference accuracies on target training sets, which is close to 50\%. This shows that domain adaptation based on discrepancy has the property to improve models' resistance toward membership inference, especially on the target.
Besides, compare to \autoref{tab:accuracies_of_classification_and_membership_inference_on_amazon_and_webcam}, membership inference accuracies on both domains are lower than the ones obtained from models that are directly trained on the corresponding domain.

Apart from membership inference, it can be observed that the gap between training accuracy and test accuracy varies with the diversity of the source and target. The test accuracy is close to the training accuracy when the target is similar (visually) to the source. Is this a factor that affects the experiment results? We exploit this in the next section.


% 评估 adversarial-based 方法
\subsubsection{Evaluation on adversarial-based domain adaptation}

Now we evaluate adversarial-based domain adaptation to investigate the effects of domain adaptation on membership inference. 
A model is firstly trained on the source domain, which is then split into two parts: 1.the feature extractor and 2.the classifier. Next, the source the feature extractor is served as the generator who keeps updating itself until the feature extracted from that target can fool the discriminator. Eventually, the updated feature extractor with the source classifier is treated as the target model. In these experiments, we use ADDA\cite{tzeng2017adversarial} as the adversarial-based domain adaptation approach.

During the experiments, we found it tough for the model to converge, especially when trained on Office 31, the losses keep fluctuating during the training phase, since the training phase is adversarial. Besides, during the training phase, two encoders for the source and the target, as well as a classifier and a discriminator are built from scratch, which is time-consuming. Moreover, the target models' performances are far from satisfactory. For example, from domain \textit{Amazon} to domain \textit{Webcam}, the target model can only achieve an accuracy of 1.2579\% on \textit{Webcam} even using ResNet-50 as backbone. Therefore, we conclude that this type of approach is not suitable to be utilized as the defense. 
However, this approach is still able to show the impact of domain adaptation on membership inference. We show the experiments on MNSIT and SVHN using AlexNet as backbone in \autoref{tab:exp02_mnist_svhn_alexnet_adda}.

\begin{table}[H]
    \centering
    \caption{Experiment results of Alexnet on MNIST and SVHN (ADDA)}
    \label{tab:exp02_mnist_svhn_alexnet_adda}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
        MNIST $\rightarrow$ SVHN & 0.9875      & 0.9883      & 0.137803    & 0.139943    & 0.502622    & 0.5148440   \\ \hline
        SVHN $\rightarrow$ MNIST & 0.903531403 & 0.8811846   & 0.735633    & 0.7426      & 0.561987    & 0.5007183   \\ \hline
        \end{tabular}%
    }
\end{table}


% 评估 reconstruction-based domain 方法
\subsubsection{Evaluation on reconstruction-based domain adaptation}  

We further evalutate on adversarial-based domain adaptation to investigate the effects of domain adapataion on membership inference. In this approachees, the whole model use a encoder to learning the shared representation of both the source and the target by multitask learning: 1. learn to classify the source correctly; 2. learn to reconstruct the target by the decoder. We choose DRCN\cite{ghifary2016deep} to conduct our experiments. We use a vallina CNN with 3 convolution layer and 2 full conection layers to test on  MNIST vs. SVHN and Office 31  Experiment results are shown in \autoref{tab:exp03_mnist_svhn}.

\begin{table}[H]
    \centering
    \caption{Experiment results of DRCN on MNSIT and SVHN}
    \label{tab:exp03_mnist_svhn}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
        MNIST $\rightarrow$ SVHN & 0.99425    & 0.993400    & 0.162838     & 0.191726    & 0.501316667 & 0.525682    \\ \hline
        SVHN $\rightarrow$ MNIST & 0.941166    & 0.914298    & 0.682617     & 0.696000    & 0.522691311 & 0.500008    \\ \hline
        \end{tabular}%
    }
\end{table}

\begin{table}[H]
    \centering
    \caption{Experiment results of DRCN on Office 31}
    \label{tab:exp03_office}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{Adapation\\direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    Amazon $\rightarrow$ DSLR   & 1.0 & 0.55        & 0.412060302 & 0.55        & \textbf{0.663072169} & \textbf{0.568492462} \\ \hline
    Amazon $\rightarrow$ Webcam & 1.0 & 0.459119497 & 0.375786164 & 0.459119497 & \textbf{0.672370645} & \textbf{0.550314465} \\ \hline
    DSLR $\rightarrow$ Amazon   & 1.0 & 0.242907801 & 0.220594763 & 0.242907801 & \textbf{0.723316583} & \textbf{0.526324239} \\ \hline
    DSLR $\rightarrow$ Webcam   & 1.0 & 0.836477987 & 0.798742138 & 0.836477987 & \textbf{0.719497487} & \textbf{0.58490566 } \\ \hline
    Webcam $\rightarrow$ Amazon & 1.0 & 0.290780142 & 0.253883711 & 0.290780142 & \textbf{0.711477987} & \textbf{0.517025762} \\ \hline
    Webcam $\rightarrow$ DSLR   & 1.0 & 0.9         & 0.891959799 & 0.9         & \textbf{0.683176101} & \textbf{0.600452261} \\ \hline
    \end{tabular}%
    }
\end{table}

As shown in \autoref{tab:exp03_mnist_svhn} to \autoref{tab:exp03_office}, it is noticeable that the accuracy of membership inference on the target is mostly lower than the source. Besides, even though a simple network cannot handle a more complex classification task like Office 31, an attacker still cannot infer the membership information from the target domain.



% 总结三个实验结果，分别是怎样的（每一小节都会提及），简述这三个结果都反映了什么.
According to the experiment results, not all the domain adaptation approaches are appropriate to defend against membership inference on the target domain, in which the discrepancy-based approaches appear to the most efficient ones. All the membership inference accuracy on the target domain are all around 0.5 to 0.55, which is much more less than the ones on the source domain and the ones of the directly trained model. In other words, we can place our private dataset as the target domain and find a relative but public dataset as the source domain so as to reduce the accuracy of membership inference on the target domain.

Three sets of experiments on MNSIT vs. SVHN present similar results. On the direction from MNIST to SVHN, not only the membership inference accuracies on target are lower than the ones on the source, but also the test accuracies are much lower than 0.5, which means the utility and privacy of these models is unacceptable. However, in the other direction, test accuracies on target ascend and membership inference accuracies drop. It reveals that the selection of source domain to the target domain is highly relative to the domain adaptation, which affects the success of membership inference attack and the test accuracy on the target domain. We explore these relations in the next section. 


% 解析来关注 source domain 的那些因素会对实验结果造成影响
\subsection{Experiments on source domain}
\label{analysis_on_source_domain}


Base on the experiment results above, we claim that in most cases, domain adaption approaches provide models with the ability to resist membership inference by learning from the shared representation of the source and target rather than directly from the target, which prevents the model from memorizing unnecessary information of the target domain (i.e. the private one). However, the effects are not stable. It's natural to take the source domain into consideration when we attempt to craft domain adaption approaches as the basis of defenses, since the target domain serves as the placeholder for a private dataset, which we avoid to manipulate. Contrary to the target domain, the source domain is the one that we can control and modify according to our needs. We ponder on factors of the source domain including: 1. the size; 2. the diversity; 3. the similarity between the source and the target. In the following experiments, we choose Office 31 as the experiment dataset. 


% 探究 source domain 大小对结果的影响
\subsubsection{Effect of the Size of Source Domain}
\label{sub:source_domain_size}
We start our exploration by raising a question: will the diverse size of source domain affact the shared representation and further influence the model's performence to resist membership inference? To seek an answer to this question, we vary the dataset size of the source domain and collect measurements the same as \Cref{sec:experiments_on_different_domain_adaptaion_approaches}. 
We choose domain \textit{Amazon} as the source and \textit{Webcam} as the target. We increase the size of the source gradually from 31 (each categoriey contains 1 sample) to 2108 (each categoriey contains 1 sample at most 68 samples) and perform trainings for 100 epochs dndividually. We show the measurements in \autoref{tab:exp03_size} and plot the accuracies of test and membership inference on the target domain in \autoref{fig:exp03_size}.

\begin{table}[H]
    \centering
    \caption{Experiment results on different sizes of source domain}
    \label{tab:exp03_size}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{size of \\ source domain }  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    31   & 1.0                   & 0.0                  & 0.316037736         & 0.270440252        & 1.0                 & 0.537735849       \\ \hline
    93   & 1.0                   & 0.684210526        & 0.555031447         & 0.622641509        & 0.914295875       &    0.516509434       \\ \hline
    186  & 0.993243243         & 0.616352201        & 0.610062893         & 0.616352201        & 0.784672831       &    0.533805031       \\ \hline
    310  & 0.991935484         & 0.685534591        & 0.682389937         & 0.685534591        & 0.713709677       &    0.52908805        \\ \hline
    465  & 1.0                   & 0.660377358        & 0.694968553         & 0.660377358        & 0.686827957       &    0.528301887       \\ \hline
    620  & 0.997983871         & 0.716981132        & 0.699685535         & 0.716981132        & 0.660282258       &    0.511006289       \\ \hline
    930  & 0.963709677         & 0.72327044         & 0.724842767         & 0.72327044         & 0.620967742       &    0.525157233       \\ \hline
    1302 & 0.91988417          & 0.710691824        & 0.746855346         & 0.710691824        & 0.588602614       &    0.521226415       \\ \hline
    1736 & 0.911078717         & 0.748427673        & 0.740566038         & 0.748427673        & 0.585183741       &    0.517295597       \\ \hline
    2108 & 0.883524442         & 0.742138365        & 0.732704403         & 0.742138365        & 0.561973664       &    0.519654088       \\ \hline
    % 2817 & 0.872727273         & 0.754716981        & 0.712264151         & 0.754716981        & 0.556520989       &    0.514937107       \\ \hline
    \end{tabular}%
    } 
\end{table}

% TODO: 采集不少于 10 个点的数据？

\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/exp03_size.pdf}
    \caption{Test accuracies and membership inference accuracies of the target domain vary under different source sizes. The membership inference accuracies keep low despite the data deficiency of the source. However, sufficient source samples are needed to increase the test accuracy on the target.}
    \label{fig:exp03_size}
\end{figure}

We can observe that with the size of the source increasing, the test accuracy on the target domain also ascends and the membership inference accuracy also decreases. It's noticeable that the drop of the membership inference accuracy is not slight since it remains low even though the size of the source is 31 only. However, in order to have a better performance on the target, sufficient data from the target is needed. 

Based on the results, we draw a conclusion that the size of the source domain does influent the success of membership inference. However, the impact is slight since the attack accuracy is close to 0.5 and flat even with the size ascending. Besides, the test accuracy on the target is proportional to the size of the source. However, the accuracy won't keep climbing but finally reach a plateau. This seems an upper bound that decided by the source domain. We question whether the constituents of the source affect this upper bound and seek to come up with an answer in the next sections. 



% 探究 source domain 多样性对结果的影响
\subsubsection{Effect of the Diversity of Source Domain}
\label{sub:source_domains_diversity}

Intuitively, the more diverse the source domain is, the more confused the shared representation is. Will it make it more difficult for an attacker to do membership inference on a model trained by this shared representation? To answer this question. we conduct another experiment to measures the success of membership inference by changing the diversity of the source domain.

To create a more diverse source domain, we mix two domains from Office 31. In other words, we choose one of the domains as the target domain and combine the rest two domains. The resulted domain is more diverse since the individuals in the domains come from different domains. Next, we measure the same metrics as before and show the results in \autoref{tab:exp03_diversity}.


\begin{table}[H]
    \centering
    \caption{Experiment results on mixed source domains}
    \label{tab:exp03_diversity}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{Adaptation \\ direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    mix $\rightarrow$ Amazon & 1.0                   & 0.992277992        & 0.634265424         & 0.640070922        & 0.58528375        & 0.501714027       \\ \hline
    mix $\rightarrow$ DSLR   & 0.823906486         & 0.784313725        & 0.854271357         & 0.83               & 0.541855204       &    0.549346734       \\ \hline
    mix $\rightarrow$ Webcam & 0.815987934         & 0.802413273        & 0.8525              & 0.8                & 0.528092006       &    0.56625           \\ \hline
    \end{tabular}%
    } 
\end{table}

As \autoref{tab:exp03_diversity} shows, the accuracies of membership inference on the target don't vary dramatically. On the contrary, when compared with ones that measured from models trained by a pure domain (shown in \autoref{tab:exp01_offcie31_resnet50}), we find that they are close to each other with a modest difference. Besides, the test accuracies on the target are inconsistent with the pure ones. These accuracies are roughly equivalent to the mean of the ones that are measured on the pure domain separately (see \autoref{tab:exp03_diversity_target}).


\begin{table}[H]
\centering
\caption{Membership inference accuracies on the target domains}
\label{tab:exp03_diversity_target}
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \diagbox{Target}{mia acc.}{Source} & Amazon      & DSLR        & Webcam      & Mix         \\ \hline
        Amazon                    & -           & 0.507515983 & 0.501553484 & 0.501714027 \\ \hline
        DSLR                      & 0.542964824 & -           & 0.551909548 & 0.549346734 \\ \hline
        Webcam                    & 0.517295597 & 0.504716981 & -           & 0.56625     \\ \hline
    \end{tabular}
}
\end{table}


\begin{table}[H]
\centering
\caption{Membership inference accuracies on the source domains}
\label{tab:exp03_diversity_source}
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \diagbox{Target}{mia acc.}{Source} & Amazon      & DSLR        & Webcam      & Mix         \\ \hline
        Amazon                 & -           & 0.64459799  & 0.625786164 & 0.58528375  \\ \hline
        DSLR                   & 0.535641603 & -           & 0.627358491 & 0.541855204 \\ \hline
        Webcam                 & 0.549949949 & 0.646055276 & -           & 0.528092006 \\ \hline
    \end{tabular}
}
\end{table}


Therefore, the mix of domains seems to bring no improvement in reducing the success of membership inference on the target. However, we do observe a decrease in membership inference accuracies on the source domain (see \autoref{tab:exp03_diversity_source}). For example, the membership inference accuracies are 0.64459799 and 0.625786164 when transferring from \textit{DSLR} or \textit{Webcam} to \textit{Amazon}. After mixing domains, the membership inference accuracy reduces to 0.58528375. Even though the source domain is not our focus, it might be of use when the privacy of the source domain is taken into consideration.


% 探究 source 和 target 的相似性对实验结果的影响
\subsubsection{Effect of the Similarity between Source Domain and Target Domain}
\label{sub:source_domains_similarity}


\begin{figure*}[ht] % ht for here,top
    \label{fig:exp03_similarity}
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/exp03_similarity.pdf}
    \caption{An image of desk lamp from original domain \textit{Webcam} and its perturbed versions from the corresponding source source domain. The main difference between the perturbed ones and the original is the brightness, contrast, gaussian noise and motion blur.}
\end{figure*}


Notice that in \Cref{sec:experiments_on_different_domain_adaptaion_approaches}, experiment results about DSLR and Webcam are appealing. No matter what adaptation direction is (\textit{DSLR} to \textit{Webcam} or \textit{Webcam} to \textit{DSLR}), test accuracy of either source domain or target domain is satisfactory (more than $90\%$) while the accuracy membership inference on the target remains low. The high test accuracy on the target domains has a connection to the source domain, which will determine the upper bound of the test accuracy on the target. Recall that in \autoref{sub:source_domain_size} where domain \textit{Amazon} is the source and \textit{Webcam} is the target, the test accuracy finally reach about 0.75 even though the source size increases.

We thus ponder the similarity between the source domain and the target domain. The similarity is defined as the overall closeness between the two domains in the human-eye level. For example, as shown in \autoref{img:office31}, the difference between Webcam and DSLR is slight. The contrast between the two domains is the light condition caused by cameras, except which the images remain the same for human eyes. 
We consider a question that: Using a similar source with one major difference such as light condition, will the resulted model preserve high test accuracy and low membership inference accuracy on the target domain? To answer this question, we crafted several source domains similar to the target domain and collect the necessary measurements by experiments.

When the source and the target have no difference except factors like light condition, crafting a similar dataset can be viewed as introducing perturbations into the target and use the perturbed target as the source.\citet{hendrycks2019benchmarking} provides a method to produce images with specific perturbations. We use their tools\footnote{https://github.com/hendrycks/robustness} to build our source domains. There are more than 15 perturbations that can be used to perturb the target domain, however in this section, we choose 4 of them, which are brightness, contrast, gaussian noise and motion blur. 

We choose \textit{Webcam} as the target domain and create 4 similar source domains mentioned with perturbations mentioned before. Their visual difference between the original one is shown in \autoref{fig:exp03_similarity}. The same as before, we apply domain adaptation from similar domains to the original domain and collect measurements of necessity. In the experiments, all the models are trained in 100 epochs with a learning rate of 0.0001. The results are shown in \autoref{tab:exp03_similarity}.

\begin{table}[H]
    \centering
    \caption{Experiment results on similar source domains}
    \label{tab:exp03_similarity}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \tabincell{c}{Adaptation \\ direction}  & \tabincell{c}{train acc.\\ on source}   & \tabincell{c}{test acc.\\ on source} & \tabincell{c}{train acc.\\ on target}  &  \tabincell{c}{test acc.\\ on target} & \tabincell{c}{mia acc.\\ on source}  &  \tabincell{c}{mia acc.\\ on target}  \\ \hline 
    Brightness $\rightarrow$  Original     & 1.0          & 1.0        & 0.993710692 & \textbf{1.0}             & 0.647798742 & \textbf{0.510220126} \\ \hline
    Contrast $\rightarrow$  Original       & 1.0          & 0.993710692 & 0.993710692 & \textbf{0.993710692} & 0.642295597 & \textbf{0.512578616} \\ \hline
    Gaussian Noise $\rightarrow$  Original & 0.998427673 & 0.974842767 & 0.988993711 & \textbf{0.974842767} & 0.626572327 & \textbf{0.522012579} \\ \hline
    Motion Blur $\rightarrow$  Original    & 1.0         & 0.993710692 & 0.995283019 & \textbf{0.993710692} & 0.663522013 & \textbf{0.512578616} \\ \hline
    \end{tabular}%
    } 
\end{table}

% 实验结果阐述
The experiments appears to be promising. It can be observed that the amaong 4 similar domains, the trained models demostrate acceptable resistence to membership inference on the target domain. Moreover, the test accuracies on the target are also close to the ones on the source, which are nearly 100\% in these cases. Hence, by crafting a similar domain from the target domain with some perturbation and utilizing it as the source domain for domain adaptation training, a trained model can not only lower the menbership inference accuracy on the target but also push the test accuracy on the target as close to the ones on the source as possible. 

Although the source domains are regarded to be public, however in a more real scenario where one may try to resist membership inference by trainig a model in this manner, the source domain cannot be public since it is created from the private target domain. A simple solution is that the souce domain is also kept secret to the public. Nevetherless, it needs further research to answer the question that whether higher success of membership inference on the crafted source will lead to information leakage on the target.


% 或许需要解释一些为什么有些数据是一模一样的（因为数据量不大，而且每一个模型所使用的数据集划分都是一样的，这是由于程序的随机种子是固定的）

==> Trashbin/Z-_abandoned_-sec5-analysis.tex <==

\section{Analysis} 
\label{sec:analysis}

% 引入，之前的实验结果看起来不错，那么为什么会有这样的效果？
% DA 是否改变了模型的行为，进而带来这种效果？
According to the experiments in the previous section, we see that by leveraging domain adaptation, a trained model demonstrates resistance to membership inference despite that the test accuracy on the target varies. An attacker can only gain accuracy at roundly between 0.5 and 0.5 in most cases, some of which are close to a random guess. Furthermore, by crafting a source domain resembles the target domain, the test accuracy can be improved while the resistance to membership inference persists, which shows the promise of adopting domain adaptation as a defense against membership inference. However, there are questions remaining. Why does the model trained by domain adaptation works? Does the domain adaptation change the behavior of a model and thus lead to membership inference resistance? 

To show the difference between a model trained with/without domain adaption, we plot the generalization error, the prediction distributions\cite{nasr2018machine} and the intermediate representations of the two models. Models trained directly on domain \textit{Webcam} from Office 31 and by domain adaptation from \textit{DSLR} to \textit{Webcam} are used, which have the same model architecture (i.e. AlexNet).



\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{paper/Figures/alys_gene_err_webcam.pdf}
    \caption{The empirical CDF of the generalization error of models across different classes on \textit{Webcam}. Curves that lean to the left show less generalization error.}
    \label{fig:alys_gene_err}
\end{figure}

\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{paper/Figures/alys_gene_err_amazon.pdf}
    \caption{The empirical CDF of the generalization error of models across different classes on \textit{Amazon}. Curves that lean to the left show less generalization error.}
    \label{fig:alys_gene_err}
\end{figure}

The generalization error on \textit{Webcam} and \textit{Amazon} between two kinds of models is shown in \autoref{fig:alys_gene_err}. The generalization error is computed as the difference between the training accuracy and the test accuracy of a model\cite{hardt2015train}. It is clearly the with domain adaptation, a model has less generalization error, indicating that the model trained by domain adaption is much likely to treat training samples and test samples equally, although the test accuracy of the domain adaptation model is lower then the traditionally-train model (for example, the test accuracy on \textit{Aamzon} is round 40\%, while the traditionally-train one reaches about 62\%). This claim can be further confirmed by the difference in prediction distributions between training data and test data.

\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/alys_ditribution_cls.pdf}
    \caption{The output distribution of two models on the training data and test data from class 7,15,18,28 in \textit{Webcam}.}
    \label{fig:alys_ditribution_cls}
\end{figure}

In \autoref{fig:alys_ditribution_cls}, we plot the prediction distributions (i.e the predictions of a model on samples from a specific class) of the two models on class 7,15,28,28. Subplots on the left-hand side are the prediction distributions of the model trained traditionally, while the right depicts the model trained with domain adaptation. In each subplot, the blur curve represents the distributions of the training data and the orange one shows the test data. Apparently, the difference between training data and test data of the model trained with domain adaptation is less than the traditional one. Consider that membership inference is performed by exploiting the inequal way that a model processes the training data and the test data, the diminishment of the difference hence reduce the success of membership inference.

To better understand how domain adaptation changes the behavior of a model and affect the success of membership inference, we demonstrate the intermediate representation of the two models and inspect the difference.


\begin{figure*}[ht] % ht for here,top
    \label{fig:alys_features}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/features.pdf}
    \caption{Intermediate features of the traiditioanal model (left) and the domain adaptaion model (right)}
\end{figure*}


As shown in \autoref{fig:alys_features}, we plot the intermediate representation\footnote{We use the output of the 5th convolution layer} of both training data and test set from \textit{Webcam} that processed by two models and use different colors for every class. It can be observed that each class forms a more compact cluster on the right (i.e the model trained by domain adaptation). More importantly, on the right-hand side, the intermediate representation of the test samples is much close to the training samples. For example, on the left side, class 15 is much more sparse. Moreover, the test samples reside almost inside the training samples on the right.
The outcome indicates that the model trained by domain adaptation does fit well on both training data and test data, in other words, the model trained by domain adaptation treats the training data and test data more equally, which makes membership inference more difficult. Since membership inference can be reckoned as building a binary classification model whose input is the output of the victim model, it becomes challenging to build a model to find a decision boundary to separate training data and test data when they are clustered closely.

Consequently, we conclude that owing to the behavior change caused by domain adaptation, the difference of the way that a model process training data and test data from the target domain is slight, and thus reduce the success of membership inference.



==> Trashbin/Z-_abandoned_sec2_5-leveraging_da_as_a_defense.tex <==
\section{DAMIA: Domain Adaptation against Membership Inference Attacks} % (fold)
\label{sec:leveraging_domain_adaptation_as_a_defense} 

In this section, we first define our threat model. Afterwards, we shed light on the idea of DAMIA, in which we leverage DA as a defense against membership inference attacks.

\subsection{Threat Model}

Our DAMIA works under the scenario where a DL model is served to the public in a MLaaS (Machine-Learning-as-a-Service) platform, and only the prediction APIs that users invoke to feed inputs the model are exposed. In such a scenario, users can collect the outputs (i.e., the prediction vectors) when the model finishes the processing, and the goal of DAMIA, as the name implies, is to defeat the membership inferring attacks. 
%After the model process the inputs, the direct outputs (i.e. the prediction vectors) are sent to the user. 
%The goal of the DAMIA is to prevent attacker from the inferring the membership of some data, even though the attacker hold the training data of the target model. 
Specifically, we make the following assumptions:

\begin{enumerate}
\item We assume that the attacker has only black-box access to the target model (which is also referred to victim model). That is, the only way an attacker can interact with the victim model is to invoke the prediction APIs and collect outputs from the victim model. 
\item We assume that the attacker knows the distribution that the training data of the victim model drawn from, 
% 关于 distribution 可以这样理解。其实就是概率论中的分布，采样全学校的C语言程序期末成绩，计算出概率密度函数，这个函数就反映了这些数据的分布，从这个分布中采样的数据是服从这个分布的。
%每一批数据背后都有对应的一个分布。我们假设假设了敌手知道 victim model 训练集的数据分布，其实就是说明敌手能够采样出和 victim 模型分布相同甚至一模一样的数据。
meaning that an attacker may obtain all the possible values in the training data that the model trained on. However, given specific data, the attacker does not know whether it is in the training dataset. Note that this assumption is also made in most of the membership inference threat model \cite{shokri2017membership, yeom2018privacy, salem2018ml}.
%of the target model, even though he/she may not know the data is for training the target model;
%\item \delete{we assume that the attacker perform membership inference using the threshold-based method
%\cite{yeom2018privacy} 
%mentioned in 
%\autoref{sec:leveraging_domain_adaptation_as_a_defense}.
%This method is effective, efficient and of simplicity.} \ZY{This is not our assumption but our experiment settings.}
\item We assume that the attacker does not aware the implementation of the target model, including the architecture, the training algorithm and the hyperparameters such learning rate and regularization values. This is reasonable because the other than model, the underingly architecture as well as the hyperparameters is usually not public in practical. 
\end{enumerate}


\ZY{No other assumptions? Can the attacker access the target domain (Yes, right?)/ source domain? }

% ================  NOTE STARTS ================  
% 同样是研究 Membership Inference Attack，《ML-Leaks: Model and Data Independent Membership Inference Attacks and Defenses on Machine Learning Models》的威胁模型描述如下：
%We deﬁne our attack model A as a supervised ML classiﬁer with binary classes (member or non-member). To train A, the adversary needs to derive the labeled training data. i.e., the ground truth membership. As mentioned in Section II, the adversary only has black-box access to the target model, i.e., she is not able to extract the membership status from the target model. Therefore, the adversary trains a shadow model [38] to mimic the behavior of the target model, and relies on the shadow model to obtain the ground truth membership to train A.
%To train the shadow model, we assume that the adversary has a dataset, denoted by D Shadow , that comes from the same underlying distribution as the training data for the target model. Note that most of the experiments by Shokri et al. [38] make the same assumption.
%We further assume that the shadow model uses the same ML algorithm and has the same hyperparameters as the target model. To achieve this in practice, the adversary can either rely on the same MLaaS provider which builds the target model or perform model extraction to approximate the target model [43], [30], [45]. Later in this section, we show this assumption can be relaxed as well.

% 2020.04.17
% ================  NOTE ENDS ================  
 
%\ZY{Give one more assumption.} 
\subsection{Overview}
% 为什么用 DA

\begin{figure}[ht]
    \label{fig:overview_of_damia}
    \centering
    \includegraphics[width=0.48\textwidth]{./Figures/DAMIA.pdf}
    \caption{The Overview of Domain Adaptation against Membership Inference Attack.}
\end{figure}

Membership inference attacks are feasible due to the fact that the model may achieve a better performance when the input is from the training dataset, which is considered as sensitive. We denote the training dataset as $D_{T}$.  Therefore, provided that a model is trained on a dataset (denoted as $D_{T}^\prime$) other than $D_{T}$, membership inference attacks against $D_{T}$ are not possible. However, a model is not trained on $D_{T}^\prime$, may not achieve the same goal in a specific task as $D_{T}$ does. For example, categorizing pictures of cat and dogs clipped from animation movies may not be preformed if the pictures of cat and dogs aforementioned were not given during the training process. Our paper is to explore a solution that may bridge the gap between $D_{T}^\prime$ and $D_{T}$ in usability, and domain adaptation appears to be a possible one. 

Domain adaptation requires one dataset from the source domain and one dataset from the target domain. Therefore, a dataset, denoted as $D_{T}^{s}$, related to $D_{T}$ is provided as the dataset from the source domain, while $D_{T}$ is in the place of the target domain. Please note that  $D_{T} \neq D_{T}^{s}$. Afterward, we adopt DA to extract a shared representation of $D_{T}^{s}$ and $D_{T}$, and the shared representation is $D_{T}^\prime$. It can be observed that $D_{T}$ is obfuscated in such a manner and membership inference attacks are not valid.  




%a model is trained by transferring the knowledge from the source domain to the target domain. \red{,in which the target domain can be incomplete.} \ZY{Why are you keep referring the target domain is incomplete? If not, what will happen then? } \red{That is, only the samples with labels in the target domain are provided to the model.}\ZY{Source domain? Or target domain without label? I am confused now.} During training, a shared representation of the two domains is extracted and used by the model for a specific task such as image classification.



%For the purpose to protect the private dataset, we applying the domain adaptation in the following way:

%Based on \autoref{sec:background}, we know that the reason why membership inference is feasible is that a trained model contains information relative to the training data, for example, the distribution of the training dataset. Consider that a DL model is essentially a mathematical model. The model may learn the distribution of the training dataset so well that when an input is out of the training dataset is fed, the model cannot process the input as good as the training data. This can be exploited to do membership inference. We try to mitigate membership inference by closing this gap. Particularly, we prevent the model from directly accessing the training dataset, which may avoid the model from fitting the training data too much, and thus the difference between the process of traning data and test data can be diminished. The problem is how to train a model without giving the model full access to the training dataset. Domain adaptation appears to be a solution. 

% 怎么用
%According to \autoref{sec:background}, in domain adaptation, a model is trained by transferring the knowledge from the source domain to the target domain, in which the target domain can be incomplete. That is, only the samples with labels in the target domain are provided to the model. During training, a shared representation of the two domains is first extracted and used by the model for a specific task such as image classification. For the purpose to protect the private dataset, we applying the domain adaptation in the following way:

\killme{
\begin{itemize}
\item[1.] we place the the training dataset of a private dataset in the target domain, whose labels are not used for training;
\item[2.] we find a public dataset relative to the private dataset, whose training dataset acts as the source domain and can be adjusted according to our needs;
\item[3.] we use domain adaptation training to train the model.
\end{itemize}
}

We demonstrate the overview of DAMIA in \autoref{fig:overview_of_damia} and interpret it in \autoref{alg:algorithm_of_DAMIA}

\ZY{Try to involve symbols instead of text solely, making the paper looks professional. }
\begin{algorithm}
    % \Kwln ~~\\ %算法的输入参数：Input
    \caption{Algorithm of MAMIA}
    \label{alg:algorithm_of_DAMIA}
    \LinesNumbered
    \KwIn{Sensitive dataset $D_{sen}$, Public dataset $D_{pub}$, Domain Adaptaion Training Algotirhm $ DA\_training(\cdot)$}
    \KwOut{trained model $M$}
    Initialize model $M$ by constructing the architecture;
    
    Initialize $DA\_training(\cdot)$ by setting the training parameters $Param_{
    train}$ such as traning epochs $e$ and learning rate $lr$;
    
    Initialize $D_{sen}$ by removing the labels;
    
    Place the $D_{sen}$ as the target domain;
    
    Place the $D_{pub}$ as the source domain;
    
    Run $DA\_training(D_{pub},D_{sen},model,Param_{train})$ to finish training.
    
\end{algorithm}



% 在所定义的 threat model 下，测量模型的 membership inference accuracy 的方法
\ZY{The following can be a part of our evaluation and should not be placed here.} 
After the model is trained, to determine whether the model resists membership inference, we use the threat model to attack the model. The attacker first feeds the models with the training data of the target domain to receive the model's outputs; in the same way, the attacker obtains the outputs of the test data. With these two kinds of outputs, the attacker uses the threshold-based method\cite{yeom2018privacy} to build a binary classifier for membership inference. And then, the accuracy of membership inference can be measure by testing the binary classifier on the training dataset and test dataset of the target domain. A membership inference accuracy close to 0.5 means the better resistance to membership inference.

Consider that: 1. there exists different types of domain adaptation to learn the shared representation, even though for the same purpose, the constructions have subtle difference\cite{wang2018deep}; 2. as a defense, the accuracy of the model should not be largely affected for the sake of resisting membership inference. Therefore, to verify the feasibility to use domain adaptation as a defense by the way we propose, in the following sections, we conduct experiments on different domain adaptation approaches to measure the membership inference accuracy and train and test accuracy on the target domain. Besides, to better demonstrate the difference between the source and the target, we also measure the source domain.


==> Trashbin/Z_abandoned_-sec3-experiment_setup.tex <==
\section{ Experiment Setup }
\label{sec:setup }


% 实验环境
\subsection{Experiment Enviroment}
We perform our experiments in a Ubuntu 16.04 server with 40 Intel(R) Xeon(R) CPU E5-2640 CPUs, 4 GTX 1080 GPUs and memory with a size of 130 GB. We use PyTorch\footnote{https://github.com/pytorch/pytorch} to build our deep learning models for evaluation.

% 实验所用的数据集 
\subsection{Datasets}
\label{sub:datasets}
We adopt typical datasets in domain adaptation to evaluate how the information of the target domain is preserved compared with the source domain. These datasets include: 1.MINST; 2.SVHN; 3.Office 31. Datasets are utilized as either source domain or target domain, training sets of each domain are used for training only and the test set is only for test. After the model is trained, we perform membership inference attacks against the model for both domains respectively and compare the inference accuracies.


\textbf{MINST vs SVHN.}
MNIST is an image dataset containing handwritten digits with an image size of $ 28 \times 28 $. All the digits are in the range of 0 to 9 and all the Figures are grayscale. MNIST dataset contains 70,000 Figures totally, in which 60,000 Figures are used as the training set and the rest are served as the test set. It's widely applied in machine learning, especially in classification tasks. 
Similar to MNIST, SVHN is also an image dataset of digits of 0 to 9 with an image size of $ 32 \times 32 $, which is separated into 3 datasets: 1. training dataset with a size of 73257; 2. test dataset with a size of 26032;  3. and the extra training dataset with a size of 531131. 
Even though two datasets are relative to digit classification, the most difference between the two datasets is that the images of SVHN are collected form street view house numbers in the real world, which means that the Figures may contain more irrelevant information about the groud-truth, or the digits in images are much more difficult to recognize. These difficulties make it harder for a model to do classification compared with MNIST (as shown in \autoref{fig:mnist_SVHN}).
In our experiments, we use the training sets of both datasets in domain adaptation training and the test sets to evaluate the performance of the trained model. 

\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/MNIST_SVHN.png}
    \caption{Figures from MNIST(left) and SVHN(right).}
    \label{fig:mnist_SVHN}
\end{figure}


\textbf{Office 31.}
Office 31\footnote{https://people.eecs.berkeley.edu/~jhoffman/domainadapt/} is a dataset about objects commonly appeared in an office setting. The dataset totally consists of 4110 images from 3 domains --- Amazon, Webcam and DSLR, each domain contains 31 categories respectively, which is designed for domain adapation. Images in the Amazon domain are collected directly from amazon.com, which are usually preprocessed so that there is only a target object remaining on a blank white background. Figures in Webcam domain and DSLR are shot by web cameras and DSLR cameras in a real-world office. The two domains are similar to each other, the most difference is the object's pose and the lighting condition. The details of Office 31 is shown in \autoref{tab:details_of_office_31}.


% 各个 domain 的组成。
\begin{table}[]
    \centering
    \caption{Details of Office 31}
    \label{tab:details_of_office_31}
    \begin{tabular}{|c|c|c|c|}
    \hline
           & total & training set (80\%) & test set (20\%) \\ \hline
    Amazon & 2817  & 2253                & 564             \\ \hline
    DSLR   & 498   & 398                 & 100             \\ \hline
    Webcam & 795   & 636                 & 159             \\ \hline
    \end{tabular}
\end{table}

\begin{figure}[ht]
    \label{img:office31}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/Office31.png}
    \caption{Bikes from 3 Domains of Office 31.}
    \label{fig:office31}
\end{figure}


% 实验所用的 membership Inference Attack
\subsection{Membership Inference Attack}
We apply the threshold-based membership inference because it shows usability, efficiency and simplicity \cite{yeom2018privacy,song2019privacy}. Explicitly, we collect a model's prediction score vectors on all the samples in the training dataset(i.e. the members) and test set(i.e. the non-members). Then a binary classifier is built by finding the best prediction score in the collected prediction score vectors as a membership threshold to achieve maximum membership inference accuracy. Any sample's prediction score that is less then the threshold will be determined as a non-member, otherwise, it will be determined as a member.

% \subsection{Metrics}


==> Trashbin/Z_abandoned_-sec4_1-evaluation_intro.tex <==

\section{ Evaluation }
\label{sec:evaluation}


We now explore analytically the performance of DAMIA. As stated above, the intuition is that DA can obfuscate sensitive datasets with a different but related dataset, generating a shared representation that shares underlying common features with the sensitive dataset, thwarting the membership inference attack. Obviously, there is a trade-off between security and usability, due to the fact that an obfuscated dataset may not achieve the same performance as the original dataset does. Given that, we attempt to answer the following three questions. 

\vspace{2mm}
\begin{tcolorbox}[label=question]
\textbf{Q1}:\textit{ Is DAMIA effective in countering membership inference attack?  
 }
 
 \textbf{Q2}:\textit{ Do all types of domain adaptation techniques have the same effects in countering membership inference attack?
 }
  \textbf{Q3}:\textit{ What are the factors that may impact the performance of DAMIA? And how could the DAMIA achieve the best performance by manipulating those factors? 
 }
\end{tcolorbox}

%We carry out the evaluation of DAMIA in this section. We first present the experiment setup in this evaluation. Then, the evaluation is completed by answering the follwoing threes questions.

 The rest of this section is organized as follows: we first present our experiment setup. Afterwards, we use three standalone subsections to evaluate different aspects of DAMIA, answering the aforementioned three questions correspondingly. 

\killme{
\begin{enumerate}
\item Q1: What's the difference between a model with/without DAMIA in the respective of membership inference?
\item  Q2: Do all types of domain main adaptation take effects for membership inference resistance?
\item  Q3: As a controllable part of DAMIA, what are the factors of the source domain that is relative to the accuracy of membership inference on the model?
\end{enumerate}
} 


%For the first question, we examine models with/without DAMIA in terms of the generalization errors, prediction distributions and intermediate representation, which show the extent of advantages that attackers can take to initiate membership inference. For the second question, we try different types of domain adaptaion approaches mentioned in \autoref{sec:background} to train the target model. Likewise, we train different target models by introducing factors of the source domain such as size, diversity and similarity between the source and target domain.

%After the models are trained, to determine whether the model resists membership inference, we use the threat model in \autoref{subsec:threat_model} to attack the models. The attacker first feeds the models with the training data of the target domain to receive the model's outputs; in the same way, the attacker obtains the outputs of the test data. With these two kinds of outputs, the attacker uses the threshold-based method\cite{yeom2018privacy} to build a binary classifier for membership inference. And then, the accuracy of membership inference can be measure by testing the binary classifier on the training dataset and test dataset of the target domain. A membership inference accuracy close to 0.5 means the better resistance to membership inference.

==> Trashbin/Z_abandoned_-sec4_2-experiment_setup.tex <==
 
\subsection{ Experiment Setup }
\label{sec:setup }


All our experiments are conducted on a Ubuntu 16.04 server with 40 Intel(R) Xeon(R) CPU E5-2640 CPUs, 4 GTX 1080 GPUs and memory with a size of 130 GB. We use PyTorch \footnote{https://github.com/pytorch/pytorch} to build our deep learning models for evaluation. The testing dataset involved in our experiments including ($i$) \texttt{MINST} (ii) \texttt{SVHN} and (iii) \texttt{Office 31}. 

Specifically, \texttt{MINST} is an image dataset containing handwritten digits with an image size of $ 28 \times 28 $. All the digits are in the range of 0 to 9 and all the images are gray-scale. \texttt{MNIST} contains 70,000 images totally, in which 60,000 images are used as the training set and the rest are served as the test set.
Similar to \texttt{MNIST}, \texttt{SVHN} is also an image dataset of digits of 0 to 9 with an image size of $ 32 \times 32 $. The training dataset contains 73257 images, in which test dataset with a size of 26032, and the extra training dataset with a size of 531131.  Some representative samples from the two datasets are shown in \autoref{fig:mnist_SVHN}. \texttt{Office 31} \footnote{https://people.eecs.berkeley.edu/~jhoffman/domainadapt/} is a dataset about objects commonly appeared in an office setting. The dataset totally consists of 4110 images from three domains --- Amazon, Webcam and DSLR, each domain contains 31 categories respectively, which is designed for domain adaptation. Images in domain \textit{Amazon} are collected directly from amazon.com, which are prepossessed so that there is only a target object in a blank white background. Images in domains \textit{Webcam} and \textit{DSLR} are shot by web cameras and DSLR (digital single-lens reflex) cameras in a real-world office. The two domains are similar to each other, the most difference is the object's pose and the lighting condition. The details of \texttt{Office 31} is shown in \autoref{tab:details_of_office_31} and the difference among the three domains are shown in \autoref{fig:office31}. Please note that all the datasets are utilized as either source domain or target domain, and are split into training sets and test sets.  


%\red{Even though two datasets are relative to digit classification, the most difference between the two datasets is that the images of SVHN are collected form the street views in the real world, which means that the images may contain more irrelevant information and the digits in images are much more difficult to recognize.  } \ZY{Do we need these?}
%\HW{intend to tell the reader that SVHN is far different from MNIST.}







% 实验环境
%\subsubsection{Experiment Enviroment}


% 实验所用的数据集 
%\subsubsection{Datasets}
%\label{sub:datasets}
%Typical datasets in domain adaptation are used in our evaluation, including: 1.MINST; 2.SVHN; 3.Office 31. Datasets are utilized as either source domain or target domain, and are split into training sets and test sets. The details of these datasets are demonstrated ensuingly.




\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/MNIST_SVHN.png}
    \caption{Figures from \texttt{MNIST} (left) and \texttt{SVHN} (right).}
    \label{fig:mnist_SVHN}
\end{figure}

% 各个 domain 的组成。
\begin{table}[ht]
    \centering
    \caption{Details of \texttt{Office-31}}
     \label{tab:details_of_office_31}
    \begin{tabular}{cccc}
    \toprule
    \textbf{Domains} & \textbf{Total Amount} & \textbf{Training Set (80\%)} & \textbf{Test Set (20\%)} \\
    \midrule
    \textbf{Amazon} & 2817  & 2253                & 564             \\
    \rowcolor{table_gray}
    \textbf{DSLR  } & 498   & 398                 & 100             \\
    \textbf{Webcam} & 795   & 636                 & 159             \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/Office31.png}
    \caption{Bikes from 3 Domains of Office 31.}
    \label{fig:office31}
\end{figure}

\killme{
% 实验所用的 membership Inference Attack
\subsubsection{Membership Inference Attack}
We apply the threshold-based membership inference because it shows usability, efficiency and simplicity \cite{yeom2018privacy,song2019privacy}. Explicitly, we collect a model's prediction score vectors on all the samples in the training dataset(i.e. the members) and test set(i.e. the non-members). Then a binary classifier is built by finding the best prediction score in the collected prediction score vectors as a membership threshold to achieve maximum membership inference accuracy. Any sample's prediction score that is less then the threshold will be determined as a non-member, otherwise, it will be determined as a member.}
% \HW{ seems vague or not clear enough, will fix it latter.}
% \ZY{Will place it to somewhere else.}
% \subsection{Metrics}


==> Trashbin/Z_abandoned_-sec4_3-q1_model_difference.tex <==
\subsection{Effectiveness }
\label{sub:effectiveness}

To \textbf{Q1}, we define the effectiveness of DAMIA as the capabilities in defending membership inference attacks. We use two models with the same architecture, i.e., ALexNet\cite{krizhevsky2012imagenet}, and adopt a few metrics to demonstrate it. The two models are: ($i$) a model trained on dataset \textit{Webcam} from \texttt{Office 31}; ($ii$) a model trained by DAMIA, in which the target domain and source domain may vary according to the specific context.  
%(In fact, the attacker may also target \textit{Webcam}, and the methodology to defend against the attack is similar.) 
During the training process, the discrepancy-based domain adaptation technique, Deep Domain Confusion\cite{tzeng2014deep} (DDC), is adopted for training DAMIA.
%\HW{Indeed, this model is utilized through the whole \textit{Q1}, while in Generalization error parts, we provide the plot of the other two models, a legacy one trained on \textit{Amazon} and a DAMIA one trained from \textit{Webcam} to \textbf{Amazon}. I should claim it in that part.}
The membership inference attack used in our experiment is a threshold-based membership inference attack introduced in \cite{yeom2018privacy,song2019privacy}. We will not provide the details of the attack due to the page limit. 


The origination of this part is as follows: Initially, we evaluate the effectiveness of DAMIA by using two legacy metrics, which will reflect the advantage of an attacker. In particular, the metrics introduced in our paper are also widely adopted in other efforts\cite{nasr2018machine,yeom2018privacy}, and these metrics are generalization error, prediction distributions. 
Further, we also introduce two novel metrics, which may also reflect the capabilities of a model in defending the membership inference attacks.  These metrics are intermediate representation and \red{advantage of membership inference}.
Please refer to the corresponding sections for the definition of each metric. 

%Afterwards, we deploy membership inference attacks against each model to confirm that whether the attack fails. 


\subsubsection{Legacy Metrics of Effectiveness} 

\textbf{Generalization Error}:  The generalization error is a metric to evaluate the performance of a model when a non-training dataset is involved. If the generalization error is low, the model can achieve a good performance, which may be close to the performance when the model tests on the training dataset. Therefore, an attacker may want to maximize the generalization error. For each dataset, we trained two models including one with DAMIA enabled, while the other one
is idle.
For the one DAMIA enabled, we first assume the attacker may want to deploy attacks against \textit{Webcam}, so that a dataset from \textit{Amazon} is used in our experiment to obfuscate \textit{Webcam}. We then assume the attacker may want to attack against \textit{Amazon}, and similarly, the \textit{Webcam} is then used to obfuscate \textit{Amazon}. 
\autoref{fig:alys_gene_err1} and \autoref{fig:alys_gene_err2} show the generalization error for \textit{Webcam} and \textit{Amazon} respectively. It can be observed that whatever the dataset is,  a model with DAMIA enabled has a lower generalization error when compared with the one without DAMIA, indicating the DAMIA is effective in defending against the membership inferences attacks.  
 

\textbf{Prediction Distributions}:  The prediction distribution is referred to the distribution of the probability of being a sample from each class \cite{nasr2018machine} (i.e., training dataset and non-training dataset). Basically, if the prediction distribution of a training dataset and that of the non-training dataset are close to each other, one cannot tell which one is which. In other words, the membership inference attack may fail in this case. The experiment procedures and dataset used are similar to the first one, and we will not go to details. 
%Similar to the first experiment, we assume that a membership inference attack is against \textit{Webcam}. we trained two models including the one with DAMIA enabled, adapting  \textit{Amazon} to obfuscate \textit{Webcam}, while the other one is idle. 
% we deploy membership inference attacks against \textit{Webcam} and \textit{Amazon}, and for each dataset,  we trained two models including the one with DAMIA enabled, while the other one is idle. 
Recall that each dataset in \texttt{Office 31} contains different categories of images. We select and plot the prediction distributions of a few categories, including desk chair (category number ``7''), mobile phone (category number ``15''), ring binder (category number ``25'') and speaker (category number ``28'').  As demonstrated in \autoref{fig:alys_ditribution_cls}, the figures on the left side show categories of the model with DAMIA enabled, while the ones on the left side that does not. It can be observed that the prediction distributions of the model with DAMIA are more approximate when compared with the one without. This will bring more challenges for an attacker whose goal is to deploy the membership inference attacks.  


 

%We deploy membership inference attacks against \textit{Webcam} and \textit{Amazon},\HW{Is it OK to say "deploy"? It's more like we assume the attack aims at \textit{Webcam} and \textit{Amazon} since we don't actually initiate the attack.} \ZY{At that moment, I was confused and did fully understand your experiment.}






%\HW{maybe we should place it in the intro part? Actually, a membership inference attack is not deployed in this part. The three metrics are more like providing fundamental reasons to why membership inference fails.}


%\red{The effectiveness of DAMIA can be evaluated by the membership inference accuracy that an attacker can achieve on the target domain. However, we intend to provide a more essential  evaluation with metrics that reflect the attacker's advantage.}

%Therefore, to evaluate the effectiveness from different aspects, we first introduce two metrics, i.e.,  generalization error, prediction distributions. Those metrics are also widely used to evaluate if the membership inference attacks are possible to be deployed against a model. 

%In particular,  Moreover, we also introduce a new metric, i.e., intermediate representation, to further confirm the effectiveness of our model. \red{The intermediate representation is the outcome of some inner layer of a DL model. Given that the function of a DL model can be regarded as a procedure of processing information layer by layer, the intermediate representation can reflect the way a model process its inputs. If the intermediate representations of training data and non-training data are distinctly different, one can easily tell training data from others. That is to say, attackers are less likely to take advantage if the intermediate representations of training and non-training data are close.}
% \HW{rewrite the third metric}
% \ZY{Overall, the descriptions are unclear and hard to follow. Can you give a new definition follow my style? What is the metric (one or two sentence is far more than enough) and what is the relationship between the metric and the attack (or defense). }

 \ZY{Please use non-training set in our paper, which is much more clear.}.\HW{will do latter} 


 
 

%To have a better understanding on how a model handles training set and non-training dataset, and how DAMIA close this gap visually, we exhibit the the intermediate representation of the two models. That is to say, we can extract outputs from an intermediate layer of the model as intermediate representations by feeding data to models and have them plotted in a 2-dimensional space after dimension reduction, from which we can immediately grasp the way a model process inputs.


%Besides, to better understand the difference, the intermediate representations of the two models are also extracted and provided, \red{which present the ways models process data}\ZY{So what?}

%\red{Essentially, a membership inference attacker take the best of the difference between how a model handles training set and non-training setThe generalization error and prediction distributions are available for a membership inference attacker to exploit \cite{nasr2018machine,yeom2018privacy}. By comparing the a model trained by DAMIA and a legacy one in terms of these two metrics, we can prove the effectiveness of DAMIA. }


%We apply the threshold-based membership inference because it shows usability, efficiency and simplicity \cite{yeom2018privacy,song2019privacy}. Explicitly, we collect a model's prediction score vectors on all the samples in the training dataset(i.e. the members) and test set(i.e. the non-members). Then a binary classifier is built by finding the best prediction score in the collected prediction score vectors as a membership threshold to achieve maximum membership inference accuracy. Any sample's prediction score that is less then the threshold will be determined as a non-member, otherwise, it will be determined as a member.

%That is, we compare the difference between models with or without DAMIA. Since the outputs of model can be leveraged to perform membership inference and the outputs are related to the generalization error, prediction distributions, we show the difference of the two models in these two angles. Besides, to better understand the difference, the intermediate representations of the two models are also extracted and shown.




\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{./Figures/alys_gene_err_webcam.pdf}
    \caption{The empirical CDF of the generalization error of models across different classes on \textit{Webcam}. \red{DAMIA use \textit{Amazon} for obfuscation.} Curves that lean to the left show less generalization error.}
    \label{fig:alys_gene_err1}
\end{figure}

\begin{figure}[ht] % ht for here,top
    \centering
    % \ZY{In figures,  D.A should be DAMIA}
    \includegraphics[width=0.45\textwidth]{./Figures/alys_gene_err_amazon.pdf}
    \caption{The empirical CDF of the generalization error of models across different classes on \textit{Amazon}. \red{DAMIA use \textit{Webcam} for obfuscation.} Curves that lean to the left show less generalization error.}
    \label{fig:alys_gene_err2}
\end{figure}

 



%\red{Since generalization error can reveal the extent to how a model overfits its training set in a proportional relation and overfitting has been proved to be highly connect to the risk of membership inference\cite{yeom2018privacy}, if a model trained with DAMIA has lower generalization error compared to a legacy one, we can confirm effectiveness of DAMIA.}

%\red{To demonstrate the difference of generalization error  between the two models, we plot the cumulative distributions of their generalization error over different classes. For every classes, we collect the training dataset accuracy and non-training dataset accuracy of the model by feeding samples from this class\cite{hardt2015train}. }
%\autoref{fig:alys_gene_err} shows the generalization error on \textit{Webcam} and \textit{Amazon} of the two models. It can be observed that with DAMIA enabled, \red{a model has a lower generalization error},\ZY{less generalization errors? less generalization error rate?} \HW{Let's say lower generalization error? Besides, should I mention that a curve leaning to the top-left corner means a lower generalization error? Although I mention it in the caption of \autoref{fig:alys_gene_err}} \red{indicating that the model is less overfitted on training data.} In other words, a model train by DAMIA is more likely to treat training samples and test samples equally. Consequently, the advantage that a attacker can take in terms of overfitting to initiate membership inference is weaken.

%\red{It should be noted that although less overfitting on training set, model trained with DAMIA has a lower test accuracy than the legacy one. We seek to address this problem in} \autoref{sub:factors_of_the_source_domain}.\ZY{We will fix this when it is the time.}

% although the test accuracy of the domain adaptation model is lower then the traditionally-train model (for example, the test accuracy on \textit{Aamzon} is round 40\%, while the traditionally-train one reaches about 62\%). 
% This claim can be further confirmed by the difference in prediction distributions between training data and test data.\ZY{So what? Why you claim that the model has a better performance in countering the MI attacks, when compared with legacy ones? You have to explain it, i.e., what is the relationship between such a generalization error and the MI attacks, otherwise, nobody can understand your paper.}

\begin{figure}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/alys_ditribution_cls.pdf}
    \caption{The output distribution of two models on the training data and test data from class 7,15,18,28 in \textit{Webcam}.}
    \label{fig:alys_ditribution_cls}
\end{figure}

  

%left depicts the prediction distributions of a legacy model, while the right depicts the one trained with DAMIA. In each subplot, the prediction distributions of training data and test data is drawn by a blur curve and an orange curve individually. We can observe that the distinguishability between prediction distributions of training and test data of the model trained by DAMIA is more slight than the legacy one, resulting a more challenging membership inference. Therefore, DAMIA still shows the effectiveness on resisting membership inference. 



%\red{A attacker commonly feed the victim  model with training data and test data and collect the direct outputs(i.e. the prediction vector) to build a binary classifier to do membership inference. If the statistical differences, e.g., the prediction distributions of the training data and test data, is indistinguishable, less advantage can be taken to perform the attack\cite{nasr2018machine}. We compute the prediction distributions of some class by feeding all the training and test samples from this class to the model to obtain their predicted results(i.e. the class that the model assigns to the sample), and calculating the ratios of the number of each predicted class to the total.}\red{In \autoref{fig:alys_ditribution_cls}, we plot the prediction distributions of the two models on class 7, 15, 25, 28 respectively. Subplots on the left depicts the prediction distributions of a legacy model, while the right depicts the one trained with DAMIA. In each subplot, the prediction distributions of training data and test data is drawn by a blur curve and an orange curve individually.We can observe that the distinguishability between prediction distributions of training and test data of the model trained by DAMIA is more slight than the legacy one, resulting a more challenging membership inference. Therefore, DAMIA still shows the effectiveness on resisting membership inference.}

\subsubsection{New Metrics of Effectiveness} 



\textbf{Intermediate Representation}: Intermediate representation reveals the way of a DL model processes its training data. Basically, a DL model will go through a feature extraction process and a classification process throughout the entire tanning, and the outputs of the feature extraction process are referred to intermediate representations, which may affect the accuracy of the classification process. Given that an attacker leverage the outputs of the classification process to derive membership inference attack, intuitively, the intermediate representation may also have an association with the success rate of deploying the membership inference attack. We conduct a similar experiment to confirm our intuition, and the intermediate representations are from the fifth convolution layer (the training process goes through multiple training layers \cite{lecun2015deep}), with their dimensionalities (i.e the number of attributes that data have)\ZY{Citation?} \HW{May replace by an explanation? } reduced to two \cite{maaten2008visualizing}.  Intermediate representations are shown in \autoref{fig:alys_features}. Samples from the same category are with the same color and the same category label, and we carefully assign all the colors to avoid the conflicts. It can be observed that, with DAMIA enabled, data of each category forms a more compact cluster, and the intermediate representations of the non-training samples are much close to the training samples.  
The result indicates that the way that the model trained by DAMIA does process the training data and non-training in a similar way, creating barriers for distinguishing training data from non-training data. In other words,   membership inference attacks are more likely to fail.

%\red{To visualize the intermediate representations of both training data and non-training data from \textit{Webcam} for these two models, we extract intermediate representations from the 5th convolution layer and have their dimension reduced to 2 using t-SNE\cite{maaten2008visualizing}.} \ZY{Too many unexplained conceptions are involved in this sentence, may I remove this}
 
 
%used internally by 
 
%will affect the accuracy of classification, also consider that attackers commonly leverage the classification output of a DL model, we claim that the intermediate representations of the training data and non-training data should reveal the advantage the attacker can take for membership inference.  

%\red{Analogous to the previous experiments, we still assume that membership inference attack aims at \textit{Webcam} and we trained the model with DAMIA enabled adapting from \textit{Amazon} to \textit{Webcam}, while the other one is directly trained on \textit{Webcam}. To visualize the intermediate representations of both training data and non-training data from \textit{Webcam} for these two models, we extract intermediate representations from the 5th convolution layer and have their dimension reduced to 2 using t-SNE\cite{maaten2008visualizing}.


 
\begin{figure*}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/features.pdf}
    \caption{Intermediate representations of \textit{Webcam} processed by the models without (left) or with (right) DAMIA enabled.}
    \label{fig:alys_features}
\end{figure*}
% \HW{rewrite the third metric}




\textbf{Advantage of an Adversary}: We now introduce a new metric to measure the advantage of an adversary who wants to deploy a membership inference attack against a model.  With insufficient advantage, the accuracy of membership inference is merely close to a random guess. 
% \HW{gonna give the metric a name soon. Maybe $Adv.$, advantage?}\ZY{Sounds good} T
Therefore, the membership inference advantage of an adversary $adv._{mi}$ can be defined as:   
$$
    adv_{mi} = = \frac{|P_{inference} - P_{random}|}{P_{random}}
$$
In particular, $P_{inference}$ represents the accuracy of membership inference for a specific adversary, while $P_{random}$ is the possibility of a random guess, which is 0.5, in that for a specific sample, the adversary without any foreknowledge may randomly output yes or no to guess whether the sample is from the training dataset. For example, when $adv._{mi} $ closes to zero, the membership inference attack merely a random guess.  Further,  to demonstrate the feasibility, we adopt the metric $adv_{mi}$  to measure the advantages in piratical and illustrate the results in \autoref{tab:adv_w_wout_DAMIA}. As expected, with DAMIA, the advantages of attackers are significantly hindered. Please note that the training process, as well as other related information of our testing models, have been introduced before, and please refer to the previous subsection for details.  

\begin{table}[H]
    \caption{Different advantages that attackers have to infer membership on \textit{Amazon} and \textit{Webcam} with/without DAMIA enabled.}
    \label{tab:adv_w_wout_DAMIA}
    \begin{tabular}{ccccc}\hline
    \toprule
    \multirow{2}{*}{\textbf{Sensitive data}} & \multicolumn{2}{c}{\textbf{Amazon}}          & \multicolumn{2}{c}{\textbf{Webcam}} \\ 
    \cmidrule{2-5}
                   & \textbf{legacy}     & \textbf{DAMIA}                   & \textbf{legacy}    & \textbf{DAMIA}          \\ 
    \midrule
    \textbf{MIA Acc.}        & 0.77324    & 0.514514926             & 0.68003    & 0.534591195    \\
    \rowcolor{table_gray}
    \textbf{$adv._{mi}$}    & 0.54648    & \textbf{0.029029852}    & 0.36006    & \textbf{0.06918239}     \\ 
    \bottomrule
    \end{tabular}
\end{table}

%It's observable that with with DAMIA enable, the advantages of attackers noticeabley descend. It also reflect the feasibility of the mertic $adv._{mi}$. Therefore, we will use this metric for the rest experiments.





% \HW{Is it OK to introduce the new metric (P-RP/RP)in the next parts, Since it is not used here?} \ZY{Try to use it here, since the entire section is talking about effectiveness, and the adv is one of the important measurements for effectiveness. For example, (assume that) you have test the adv on all the three models, and what you can do is to move one of the experiment as well as its result in this part. I member that you were using discrepancy-based domain adaptation technique for this part, right? You may want to put the related content here. }
% \ZY{Rewrite the third metric and try to use ``my style''. }








==> Trashbin/Z_abandoned_-sec4_4-q2_different_approaches.tex <==
\subsection{Performance of different domain adaptation approaches}
\label{sub:feasibility_of_different_domain_adaptation_approaches}

To \textbf{Q2}, we explore if the use of a different domain adaptation technique will affect the performance of DAMIA. To this end, we train DAMIA with all the three approaches introduced in Section \ref{sec:background} respectively, and evaluate the corresponding performance of each model in terms of defending against membership inference attack. As discussed before, using advantage $adv_{mi}$ is a simple but effective way to evaluate if the membership inference attacks are possible. Therefore, we will continue using this metric in the rest of this section.  



% In this section, we conduct experiments to verify whether different domain adaption approaches are feasible to be utilized in DAMIA, which covers three types of domain adaptation approaches mentioned in \autoref{background}.
% \HW{gonna give the metric a name soon. Maybe $$adv_{mi}$$, advantage?}
% \red{We introduce a new metric $$adv_{mi}$_{mi}$ of measuring the advantage that attackers have in membership inference to show the feasibility of different domain adaptation approaches for DAMIA, which primarily focus on the membership inference accuracy. We give the definition as follows.
% $$
%     $adv_{mi}$_{mi} = = \frac{|P_{inference} - P_{random}|}{P_{random}}
% $$
% In the equation, $P_{inference}$ stands for the possibility for correctly inferring membership, which can be represented by the accuracy of membership inference, while $P_{random}$ is the possibility to randomly guess the membership, which equals to 0.5. $$adv_{mi}$_{mi} = 0 $ means the membership inference is merely a random guess while $$adv_{mi}$_{mi} = 1$ means a attacker can accurately infer membership with a probability of 100\%.
% }
% \red{Since we are verifying on the feasibility of different domain adaptation approaches for DAMIA, we primarily focus on the membership inference accuracy on the target domain. The goal is that the membership inference accuracy can be close to 0.5.}

 

% In the experiments, we datasets are shown in \autoref{sub:datasets} to train models and concentrate on the accuracy of membership inference and test accuracy on the target domain.


% 评估 discrepancy-based 方法
\textbf{Discrepancy-based Domain Adaptation}: We evaluate the feasibility for DAMIA that is trained via discrepancy-based domain adaptation approaches. Similar to the previous experiment, DDC (deep domain confusion\cite{tzeng2014deep} is adopted. We then deploy membership inference attacks against MNIST, SVHN and the three datasets in Office-31. To eliminate the impact of the architecture of a DL model, we use AlexNet and ResNet-50\cite{he2016deep} as the backbones of the models respectively and have them trained for 150 epochs to make sure that they are converged. The experiments are shown in \autoref{tab:exp01_mnist_svhn_alexnet} to \autoref{tab:exp01_offcie31_resnet50}. It can be observed DAMIA work against membership inference attacks effectively despite the different architectures.  





%\red{As shown in \autoref{tab:exp01_offcie31_alexnet} to \autoref{tab:exp01_mnist_svhn_resnet50}, we observe that no matter what architecture the model adopts, the advantage on the target domains are mostly close to 0, that is, the membership inference accuracy is close to a random guess. This reveals that discrepancy-based domain adaptation is available for DAMIA.}

% Besides, compare to \autoref{tab:accuracies_of_classification_and_membership_inference_on_amazon_and_webcam}, membership inference accuracies on both domains are lower than the ones obtained from models that are directly trained on the corresponding domain.

%\delete{Apart from membership inference accuracy, it can be observed that the test accuracy is close to the training accuracy when the target is similar visually to the source, for example, from  Webcam to  DSLR  and vice versa. Is this a factor that affects the experiment results? We leave it as a factor to be explored in    .} \ZY{We do not need it as of now, which may confuse the reviewers and our readers. }



% \HW{seems that the data about the source should be removed? Seems irrelative to our goal? } \ZY{Sounds good} \HW{will do soon}
\begin{table} 
    \centering
    \caption{Experiment results of AlexNet on MNSIT and SVHN}
    \label{tab:exp01_mnist_svhn_alexnet}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
        \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
        \textbf{MNIST} $\rightarrow$ \textbf{SVHN}  & 0.212566717 & 0.224953903  & \textbf{0.503727767} & \textbf{0.007455534} \\ 
        \rowcolor{table_gray}
        \textbf{SVHN} $\rightarrow$ \textbf{MNIST}  & 0.76805     & 0.7702       & \textbf{0.503108333} & \textbf{0.006216666} \\ 
        \bottomrule 
        \end{tabular}%
    }
\end{table}

\begin{table} 
    \centering
    \caption{Experiment results of AlexNet on Office 31}
    \label{tab:exp01_offcie31_alexnet}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    
    \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
    \textbf{Amazon} $\rightarrow$ \textbf{DSLR}   & 0.447236181 & 0.46         & \textbf{0.528492462} & \textbf{0.056984924} \\ 
    \rowcolor{table_gray}
    \textbf{Amazon} $\rightarrow$ \textbf{Webcam} & 0.501572327 & 0.459119497  & \textbf{0.534591195} & \textbf{0.06918239} \\ 
    \textbf{DSLR} $\rightarrow$ \textbf{Amazon}   & 0.407900577 & 0.416666667  & \textbf{0.510169656} & \textbf{0.020339312} \\ 
    \rowcolor{table_gray}
    \textbf{DSLR} $\rightarrow$ \textbf{Webcam}   & 0.938679245 & 0.93081761   & \textbf{0.522012579} & \textbf{0.044025158} \\ 
    \textbf{Webcam} $\rightarrow$ \textbf{Amazon} & 0.375055482 & 0.372340426  & \textbf{0.514514926} & \textbf{0.029029852} \\ 
    \rowcolor{table_gray}
    \textbf{Webcam} $\rightarrow$ \textbf{DSLR}   & 0.929648241 & 0.91         & \textbf{0.544296482} & \textbf{0.088592964} \\ 
    \bottomrule 
        \end{tabular}%
    } 
\end{table}


\begin{table} 
    \centering
    \caption{Experiment results of ResNet-50 on MNSIT and SVHN}
    \label{tab:exp01_mnist_svhn_resnet50}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
        
        \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
        \textbf{MNIST} $\rightarrow$ \textbf{SVHN}  & 0.219173594 & 0.227566073 & \textbf{0.511505038} &\textbf{0.023010076} \\ 
        \rowcolor{table_gray}
        \textbf{SVHN} $\rightarrow$ \textbf{MNIST}  & 0.778966667 & 0.7844      & \textbf{0.500133333} &\textbf{0.000266666} \\ 
        \bottomrule 
        \end{tabular}%
    }
\end{table}

\begin{table} 
    \centering
    \caption{Experiment results of ResNet-50 on Office 31}
    \label{tab:exp01_offcie31_resnet50}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    
    \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
    \textbf{Amazon} $\rightarrow$ \textbf{DSLR}   & 0.733668342 & 0.68         & \textbf{0.542964824} & \textbf{0.085929648} \\ 
    \rowcolor{table_gray}
    \textbf{Amazon} $\rightarrow$ \textbf{Webcam} & 0.721698113 & 0.761006289  & \textbf{0.517295597} & \textbf{0.034591194} \\ 
    \textbf{DSLR} $\rightarrow$ \textbf{Amazon}   & 0.625832224 & 0.675531915  & \textbf{0.507515983} & \textbf{0.015031966} \\ 
    \rowcolor{table_gray}
    \textbf{DSLR} $\rightarrow$ \textbf{Webcam}   & 0.962264151 & 0.981132075  & \textbf{0.504716981} & \textbf{0.009433962} \\ 
    \textbf{Webcam} $\rightarrow$ \textbf{Amazon} & 0.628051487 & 0.663120567  & \textbf{0.501553484} & \textbf{0.003106968} \\ 
    \rowcolor{table_gray}
    \textbf{Webcam} $\rightarrow$ \textbf{DSLR}   & 0.992462312 & 0.99         & \textbf{0.551909548} & \textbf{0.103819096} \\ 
    \bottomrule 
        \end{tabular}%
    }
\end{table}

 
% 评估 adversarial-based 方法
\textbf{Adversarial-based Domain Adaptation}:  
We evaluate the feasibility for DAMIA that is trained via adversarial-based domain adaptation approaches. Similar to the first experiment, we deploy membership inference attacks against MNIST, SVHN and the three datasets in Office-31. AlexNet and ResNet-50\cite{he2016deep} are severed as the backbones of the models respectively. The adversarial-based domain adaptation approach used in the experiment is ADDA (i.e. Adversarial Discriminative Domain Adaptation) \cite{tzeng2017adversarial}.  It can be observed that DAMIA work against membership inference attacks effectively in \autoref{tab:exp02_mnist_svhn_alexnet_adda}.
% \ZY{Figures or Tables?} 
Unfortunately,  the performances is not as good as we expected. For example, when \textit{Amazon} is adopted to obfuscate \textit{Webcam},  the accuracy of \textit{Webcam} is down to 1.2579\%. 
\red{Likelise, when \textit{DSLR} is adopted to obfuscate \textit{Webcam}, the accuracy is only 6.918239\%, even using ResNet-50 as the backbone, which is much deeper than AlexNet (i.e. has more layers) and should have a better capacity to learning representations\cite{sun2016deep}.} 
% \ZY{Why uses ResNet-50 as backbone may achieve better performance than expected? Some explanation should be help. }
We also find that the procedures of training DAMIA via adversarial-based domain adaptation approaches are sophisticated, in that there are four models are involved. Given its unsatisfactory performance, we argue that it is not recommended to train DAMIA via that type of approach. 

 


 
%\red{In their implementation, a DL model is split into two parts: (i) the feature extractor and (ii) the classifier. The DL model is first trained on the source domain. After the training is finished, a GAN will be established by the feature extractor along with a new-defined binary classifier, in which the feature extractor will be used to extract features from the target domain, and the binary classifier acts as a discriminator to distinguish whether the extracted belongs to the source or the target.} \HW{may move it to Section Background}
% A model is firstly trained on the source domain, which is then split into two parts: 1.the feature extractor and 2.the classifier. Next, the source the feature extractor is served as the generator who keeps updating itself until the feature extracted from that target can fool the discriminator. Eventually, the updated feature extractor with the source classifier is treated as the target model. In these experiments, 

\begin{table} 
    \centering
    \caption{Experiment results of ADDA on MNIST and SVHN}
    \label{tab:exp02_mnist_svhn_alexnet_adda}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
        
        \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
        \textbf{MNIST} $\rightarrow$ \textbf{SVHN}   & 0.137803    & 0.139943  & \textbf{0.5148440} & \textbf{0.029688}   \\ 
        \rowcolor{table_gray}
        \textbf{SVHN} $\rightarrow$ \textbf{MNIST}   & 0.735633    & 0.7426    & \textbf{0.5007183} & \textbf{0.0014366}   \\ 
        \bottomrule 
        \end{tabular}%
    }
\end{table}


% 评估 reconstruction-based domain 方法
\textbf{Reconstruction-based Domain Adaptation}: We further evaluate the feasibility of DAMIA that is trained via reconstruction-based domain adaptation approaches. We deploy membership inference attacks against \texttt{MNIST}, \texttt{SVHN} and the three datasets in \texttt{Office-31}. We choose DRCN (i.e. Deep Reconstruction Classification Networks) \cite{ghifary2016deep} to conduct our experiments. For MNIST and SVHN, we select a vallina CNN with three convolution layers and two fully connected layers as the backbone of the model. Again, we use AlexNet as the backbone for Office 31. Experiment results are shown in \autoref{tab:exp03_mnist_svhn} and \autoref{tab:exp03_office}. Similarly, the advantage for an attacker is approaching zero, indicating that DAMIA work against membership inference attacks effectively. 




\red{Among the three approaches, the discrepancy-based approaches appear to the most efficient ones.}\ZY{This one sholud go to introuduction.}\HW{got it. will move it to intro once the intro is refined.}

\begin{table} 
    \centering
    \caption{Experiment results of DRCN on MNSIT and SVHN}
    \label{tab:exp03_mnist_svhn}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
        
        \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
        \textbf{MNIST} $\rightarrow$ \textbf{SVHN}   & 0.162838     & 0.191726  & \textbf{0.525682} & \textbf{0.051364}    \\ 
        \rowcolor{table_gray}
        \textbf{SVHN} $\rightarrow$ \textbf{MNIST}   & 0.682617     & 0.696000  & \textbf{0.500008} & \textbf{0.000016}    \\ 
        \bottomrule 
        \end{tabular}%
    }
\end{table}

\begin{table} 
    \centering
    \caption{Experiment results of DRCN on Office 31}
    \label{tab:exp03_office}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    
    \toprule
        \tabincell{c}{\textbf{Adapation}\\ \textbf{Direction}}    & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\  
        \midrule
    \textbf{Amazon} $\rightarrow$ \textbf{DSLR}   & 0.412060302 & 0.55        & \textbf{0.568492462} & \textbf{0.136984924} \\ 
    \rowcolor{table_gray}
    \textbf{Amazon} $\rightarrow$ \textbf{Webcam} & 0.375786164 & 0.459119497 & \textbf{0.550314465} & \textbf{0.10062893} \\ 
    \textbf{DSLR} $\rightarrow$ \textbf{Amazon}   & 0.220594763 & 0.242907801 & \textbf{0.526324239} & \textbf{0.052648478} \\ 
    \rowcolor{table_gray}
    \textbf{DSLR} $\rightarrow$ \textbf{Webcam}   & 0.798742138 & 0.836477987 & \textbf{0.58490566 } & \textbf{0.16981132} \\ 
    \textbf{Webcam} $\rightarrow$ \textbf{Amazon} & 0.253883711 & 0.290780142 & \textbf{0.517025762} & \textbf{0.034051524} \\ 
    \rowcolor{table_gray}
    \textbf{Webcam} $\rightarrow$ \textbf{DSLR}   & 0.891959799 & 0.9         & \textbf{0.600452261} & \textbf{0.200904522} \\ 
    \bottomrule 
        \end{tabular}%
    }
\end{table}






 

==> Trashbin/Z_abandoned_-sec4_5-q3_factors_of_source.tex <==
\subsection{Factors that Affects the Usability}
\label{sub:factors_of_the_source_domain}


In the previous section, our experiment shows that  DAMIA work against membership inference attacks effectively despite the approaches. However, some of the approaches may not have a good accuracy, which hurts the usability of the original dataset. Therefore, in this section, we want to explore the factors that may affect the usability of DAMIA, which is the answer to \textbf{Q3}.  Recall that we are using dataset in the source domain to obfuscate dataset in the target domain, and therefore, we can only manipulate dataset in the source domain.  Further, we select a few factors including size, diversity and similarity that may have impacts on the usability, and adjust the dataset using those factors accordingly to see what the impacts are. Assume that source domain consists of $n$ datasets which are denoted as $D_{source} = (d_1, d_2,..., d_{n})$, where $d_{i}$ is referred to each dataset of the source domain. Particularly, we list those factors below: 
\begin{itemize}
\item \textbf{Size}.  We define the size of the source domain $D_{source} $ as follows:  
$$
    size(D_{source}) = \sum_{i=1}^{n} |d_{i}|
$$.
\item \textbf{Diversity}. The diversity is defined as the the amount of datasets involved in the source domain, which can be denoted as:
$$
    diversity(D_{source}) = |D_{source}|
$$
\item \textbf{Similarity}.  
To measure the similarity between domains, we first calculate the norm of a domain $\|D_{i}\|$ by calculating the average of all the samples in $D_{i}$, which can be regarded as a representative of the domain. Since we focus on image datasets, the representatives are essentially images. The similarity between domains is further defined as the similarity between the representatives of each domain.
To this end, we use perceptual hashing\cite{zauner2010implementation} to generate the fingerprints (i.e. a hash value) for each representative, denoted as $phash(\|D_{i}\|)$. By perceptual hashing,
%images are hashed into a fix-length binary array which keeps the correlations between images. In other words, 
if two images are perceptually identical, the difference between their fingerprints is modest\cite{zauner2010implementation}. Therefore, the similarity between domains are reflected by the difference between the fingerprints of their representatives. Formally, the similarity can defined as follows:
 
 
\begin{footnotesize}
 
$$
    similarity = 1 - \frac{phash(\|D_{source}\|) - phash(\|D_{target}\|) }{len(phash(\|D_{source}\|))}
$$
 
\end{footnotesize}
\ZY{When we place a figure/table, we usually do not use the parameter ``H'', meaning that you require the figure/table should not go somewhere else. Basically, the system will handle and manage the space issues for us if we do not require some figure must be located somewhere. Last time, the extra space is caused by that.  }
\HW{Will remove the parameter "H" later.}

% \HW{Please try this time. }
% where the \red{norm} \ZY{???} of the domain is defined as the average image of all the images in that domain whose pixels are the average of all the pixels in the same positions across all the images, and $phash$ is perceptual hashing\cite{zauner2010implementation}. By perceptual hashing, images are hashed into a fix-length binary array, and the correlations between images are also kept in these hash values. In other words, if two images are perceptually identical, the difference between the $phash$ values of the two images is small, resulting in a high similarity. \ZY{This paragraph is not clear. }
\end{itemize}
 

In the following experiments, we select Office 31 as the experiment dataset and discrepancy-based domain adaptions for DAMIA. Also, AlexNet is adopted as the the backbone of the model.

 


%\red{Consider that, as a defense, apart from shield the mode from membership inference, DAMIA should preserve the accuracy on that target domain as high as possible.Based on the experiments in this parts, we reckon that the selection of source domain to the target domain is highly relative to DAMIA, which affects the success of membership inference attack and the test accuracy on the target domain. For example, in the case of MNIST v.s. SVHN, the test accuracies on the target domain are far from satisfactory, while in the opposite direction, the test accuracy is more acceptable. Same phenomena appear in the case of using Office 31. This drive us to explore factors of the source domain that may affect the attacker's advantage and model's test accuracy on the target domain.} \HW{seems better to place it in the next part?}



%To \textbf{Q3}, we intend to explore factors of the source domain, which may have impacts on the membership inference accuracy and the test accuracy. We ponder factors of the source domain including: 1. the size; 2. the diversity; 3. the similarity between the source and target domains. 
%We give definitions to these three factors as follow.
\killme{

Supposed that a dataset of the source domain is denoted $d_{i}$, and the source domain consisting of $n$ datasets is denoted as $D_{source} = (d_1,d_2,...,d_{n})$, then the size of the source domain is defined as :
$$
    size(D_{source}) = \sum_{i=1}^{n} |d_{i}|
$$
}






%Note that apart from the metric $adv.$ defined in \textbf{Q2} is used here, we also focus the test accuracy on the source, and AlexNet is adopted as the the backbone of the model.


% 探究 source domain 大小对结果的影响

\textbf{Size}: In our experiment, we use \textit{Amazon} to obfuscate \textit{Webcam}. Particularly, we want to explore how does the size of dataset in source domain (i.e., \textit{Amazon}) affect the usability of the generated model. To this end, we gradually increase the size of each category in \textit{Amazon} from 1 to 68. Recall that \textit{Amazon} includes 31 categories in total, and therefore, the size of the source domain goes from 31 to 2108. For each dataset with the specific size, we train the model for 100 epochs to minimize the impacts of errors. We then test the accuracy of the trained model. Provided that the obfuscated model can achieve a high accuracy, the usability of the model is not hindered. Moreover, changing the size of the dataset should not impair the effectiveness. Therefore, we also deploy the membership inference attacks against the trained model.  \autoref{fig:exp03_size} shows the result.  It can be observed that a increased size of a dataset in source domain has negative impacts on the advantages of membership inference attacks slightly. This is reasonable since a lager dataset provides more samples for the model to perform the obfuscation. However, it can also be observed that even a dataset with a small size such as the one that has only 31 samples, also has an excellent effectiveness. On the hand, it can also be observed that a dataset with more samples has positive impacts on the usability.  
 
 
 %We can observe that with the size of the source domain increasing, the membership inference advantage decreases. It's surprising that the advantage of membership inference remains low even though the size of the source is 31 only. However, in order to have a better performance on the target, sufficient data from the target is needed. It's noticeable that the test accuracy on the target domain will ascends as the size of the source domain increases according to \autoref{fig:exp03_size}. Based on the results, we draw a conclusion that the size of the source domain does influence DAMIA in terms of membership inference even thought the impact is slight since the advantage is merely 0 even with a small size.  Nevertheless, size have great impact on the test accuracy on the target domain, whose relationship is proportional. However, the accuracy won't keep climbing but finally reach a plateau. This give us a insight that an upper bound of test accuracy is decided by the source domain. We seek to increase this bound in the following sections.
 

\begin{table} 
    \centering
    \caption{Experiment results on different sizes of the source domain}
    \label{tab:exp03_size}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    \tabincell{c}{\textbf{Size of}\\ \textbf{Source Domain} }   & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\ 
    \midrule
    \textbf{31  }  & 0.316037736   &  \textbf{0.270440252}   &  \textbf{0.537735849} & \textbf{0.075471698}      \\ 
    \rowcolor{table_gray}
    \textbf{93  }  & 0.555031447   &  \textbf{0.622641509}   &  \textbf{0.516509434} & \textbf{0.033018868}      \\ 
    \textbf{186 }  & 0.610062893   &  \textbf{0.616352201}   &  \textbf{0.533805031} & \textbf{0.067610062}      \\ 
    \rowcolor{table_gray}
    \textbf{310 }  & 0.682389937   &  \textbf{0.685534591}   &  \textbf{0.52908805 } & \textbf{0.0581761}        \\ 
    \textbf{465 }  & 0.694968553   &  \textbf{0.660377358}   &  \textbf{0.528301887} & \textbf{0.056603774}      \\ 
    \rowcolor{table_gray}
    \textbf{620 }  & 0.699685535   &  \textbf{0.716981132}   &  \textbf{0.511006289} & \textbf{0.022012578}      \\ 
    \textbf{930 }  & 0.724842767   &  \textbf{0.72327044 }   &  \textbf{0.525157233} & \textbf{0.050314466}      \\ 
    \rowcolor{table_gray}
    \textbf{1302}  & 0.746855346   &  \textbf{0.710691824}   &  \textbf{0.521226415} & \textbf{0.04245283}       \\ 
    \textbf{1736}  & 0.740566038   &  \textbf{0.748427673}   &  \textbf{0.517295597} & \textbf{0.034591194}      \\ 
    \rowcolor{table_gray}
    \textbf{2108}  & 0.732704403   &  \textbf{0.742138365}   &  \textbf{0.519654088} & \textbf{0.039308176}      \\ 
    \bottomrule
    \end{tabular}%
    } 
\end{table}



\begin{figure}  % ht for here,top
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/exp03_size.pdf}
    \caption{Curves of test accuracies and membership inference accuracies of the target domain under different sizes the source domain. The membership inference accuracies keep low despite the deficient size of the source. However, sufficient source samples are needed to increase the test accuracy on the target.}
    \label{fig:exp03_size}
\end{figure}




% 探究 source domain 多样性对结果的影响
% \subsubsection{Effect of the Diversity of Source Domain}
% \label{sub:source_domains_diversity}

\textbf{Diversity}: We want to explore how does the diversity of the dataset in the source domain affects the usability of the model trained by DAMIA. Therefore, we modify the diversity of datasets in source domain, and observe if the usability changes. Recall that there are three domains in \texttt{Office-31} including \texttt{Amazon}, \texttt{DSLR} and  \texttt{Webcam}.  We modify the diversity the datasets by ``mixing'' two of them together. For example,  \texttt{Mix(Amazon $\oplus$ DSLR)}  is referred to a new dataset that contains all the samples from the dataset \texttt{Amazon} and all samples from the dataset \texttt{DSLR}. \ZY{Check and see if you need to update our table.} Next, we use the mixed dataset to obfuscate the left one that is not involved in the mixing process. Similarly, all the models involved are trained for 100 epochs to minimize errors. We test the usability afterwards and deploy membership inference attacks against those models.  Results of diversity of 2 are illustrated in \autoref{tab:exp03_diversity}, and we compare the accuracy of different diversities  (i.e., diversity equals 1 and diversity equals 2 \footnote{For source domains consisting of 1 dataset, their diversity is: $diversity(D_{source}) = |D_{source}| = |(d_1)| = 1$, such source domain may be $D_{source} = (d_{Amazon})$. For source domains consisting of 2 datasets, their diversity is: $diversity(D_{source}) = |D_{source}| = |(d_1,d_2)| = 2$, such source domain may be $D_{source} = |(d_{Amazon},d_{DSLR})|   $.}) in \autoref{tab:exp03_diversity_target_test_acc} for better illustration. 
From the comparison, we see the diversity has a limited contribution to the usability. When diversity increases, the test accuracy \red{does not always proportionally ascend and may drop. For example, the test accuracy of the model using \texttt{DSLR} to obfuscate \texttt{Webcam} is higher than the one using \texttt{Mix(Amazon $\oplus$ DSLR)} for obfuscation.} \ZY{ test accuracy or accuracy? The term used in our paper should be consistent.} \HW{prefer test accuracy, since in ML, training accuracy and test accuracy are separated. The term "accuracy" may be confusing. Will check the use of this term throughout the paper later. } \ZY{What is the result? I do not understand the table.} 
\HW{Since this subsession is for usability evaluation, 
I compare the test accuracies of diversity of 1 and 2 in \autoref{tab:exp03_diversity_target_test_acc}, and to further show the limited contribution of diversity, I also show the $adv_{mi}$ of diversity of 1 and 2 in \autoref{tab:exp03_diversity_target_adv}.} \red{Likewise}, as shown in \autoref{tab:exp03_diversity_target_adv}, the comparison on the advantages of membership inference attacks with different diversities indicates that a larger diversity impairs the effectiveness of DAMIA. Therefore, DAMIA does not have advantages to be adopted to a dataset with a a large diversity. 

 
% the advantage of membership inference on the target domain don't vary dramatically and may even increase the advantage, suggesting that diversity seems have little effect on DAMIA for defending membership attacks. 






% \textbf{Diversity}:  We continue our exploration by raising another question: will it make it more difficult for an attacker to do membership inference if the source domain in DAMIA is more diverse? To answer this question, we conduct another experiment to measures the success of membership inference by changing the diversity of the source domain. \ZY{Can you rewrite the second part use my style. } 

% Limited by the dataset Office 31, we evaluate diversity of 2. To create a more diverse source domain, we mix two domains from Office 31. In other words, we choose one of the domains as the target domain and combine the rest two domains to be the source. Still, models are trained for 100 epochs in this experiment. To better compare DAMIA of different diversity in terms of resisting membership inference, we show the membership inference advantages of diversity 2 and diversity of 2. 


\begin{table}[H]
    \centering
    \caption{Experiment results on mixed source domains}
    \label{tab:exp03_diversity}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    \tabincell{c}{\textbf{Adaptation} \\ \textbf{Direction}}   & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\ 
    \midrule
    \textbf{Mix} $\rightarrow$ \textbf{Amazon}  & 0.634265424   & \textbf{0.640070922}  & \textbf{0.501714027} & \textbf{0.003428054} \\ 
    \rowcolor{table_gray}
    \textbf{Mix} $\rightarrow$ \textbf{DSLR  }  & 0.854271357   & \textbf{0.83       }  & \textbf{0.549346734} & \textbf{0.098693468} \\ 
    \textbf{Mix} $\rightarrow$ \textbf{Webcam}  & 0.8525        & \textbf{0.8        }  & \textbf{0.56625    } & \textbf{0.1325}      \\ 
    \bottomrule
    \end{tabular}%
    } 
\end{table}

\begin{table}[H]
\centering
\caption{  Test accuracies on the target domains. The diversity of Mix is 2.}
\label{tab:exp03_diversity_target_test_acc}
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{ccccc}
        \toprule
        \diagbox{\textbf{Target}}{\textbf{Test Acc.}\\ \textbf{on Target}}{\textbf{Source}} & \textbf{Amazon}      & \textbf{DSLR  }      & \textbf{Webcam}      & \textbf{Mix}        \\ 
        \midrule
        \textbf{Amazon}                      & -           & 0.407900577 & 0.375055482 & \textbf{0.64007092}  \\ 
        \rowcolor{table_gray}
        \textbf{DSLR}                        & 0.46        & -           & 0.929648241 & \textbf{0.83}       \\ 
        \textbf{Webcam}                      & 0.459119497 & 0.938679245 & -           & \textbf{0.80}       \\ 
        \bottomrule
    \end{tabular}
}
\end{table}

\begin{table}[H]
\centering
\caption{  Membership inference advantages on the target domains. The diversity of Mix is 2.\ZY{The table is confusing to read and will check all tables and figures after I am done. }}
\label{tab:exp03_diversity_target_adv}
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{ccccc}
        \toprule
        \diagbox{\textbf{Target}}{\textbf{$adv_{mi}$}}{\textbf{Source}} & \textbf{Amazon}      & \textbf{DSLR  }      & \textbf{Webcam}      & \textbf{Mix}        \\
        \midrule
        % Amazon                    & -           & 0.507515983 & 0.501553484 & 0.501714027 \\ \hline
        % DSLR                      & 0.542964824 & -           & 0.551909548 & 0.549346734 \\ \hline
        % Webcam                    & 0.517295597 & 0.504716981 & -           & 0.56625     \\ \hline
        \textbf{Amazon}                    & -           & 0.015031966 & 0.003106968 & \textbf{0.003428054}  \\ 
        \rowcolor{table_gray}
        \textbf{DSLR}                      & 0.085929648 & -           & 0.103819096 & \textbf{0.098693468}  \\ 
        \textbf{Webcam}                    & 0.034591194 & 0.009433962 & -           & \textbf{0.1325}    \\ 
        \bottomrule
    \end{tabular}
}
\end{table}

  

% Results are illustrated in \autoref{tab:exp03_diversity} and \autoref{tab:exp03_diversity_target}. Out of our expectation,  the advantage of membership inference on the target domain don't vary dramatically and may even increase the advantage, suggesting that diversity seems have little effect on DAMIA for defending membership attacks. 

\HW{maybe should place this part in disscussion? Or maybe I should just delete it.}
% 对于 source domain，有意料之外的效果, 在 source 上的 adv 下降了。
% 这里想表达的是，在实验的过程中，有一个无关文章核心的观察结果。就是说，尽管我们在实验上观察到 diversity 的变化对 DAMIA 的作用有限（无论是 effectiveness 还是 usability）。但是在实验中观察到，对于用来起混淆作用的 source domain，当我们将 diversity 提高之后，这种提高使得对 source domain 的成员推断攻击优势下降了（当然，我们之前只关注 target domain 上的成员推断攻击优势，因为是核心所在）。如果对 source domain 的隐私有所要求的话, DAMIA 也会有点作用，通过提高 diversity。可能也可以拓展其应用面。
\red{However, we observe that, for the source domain, the advantage of membership inference does drop when the diversity of the source increase from 1 to 2. For example, the membership inference advantage are 0.28919598 and 0.251572328 when adapting from \textit{DSLR} or \textit{Webcam} to \textit{Amazon}. After mixing domains, the membership inference accuracy reduces to 0.1705675. Even though the source domain is not our focus, it might be of use when the privacy of the source domain is taken into consideration.} \ZY{I am confused here. What do you mean? Can you explain it with Chinese? In our experiment, the dataset in source domain does not have another dataset involved that may obfuscate it, and its only functionality is to obfuscate the dataset in the target domain. Obviously, the source domain will not have any impact on its usability, so what are you argue for.  } \HW{try to claim the purpose of this part in Chinese. I put the claim in comments, please read it and see whether it helps for better understanding.}



\begin{table}[H]
\centering
\caption{ Membership inference advantages on the source domains. The diversity of Mix is 2.}
\label{tab:exp03_diversity_source}
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{ccccc}
        \toprule
        \diagbox{\textbf{Target}}{\textbf{$adv_{mi}$}}{\textbf{Source}} & \textbf{Amazon}      & \textbf{DSLR  }      & \textbf{Webcam}      & \textbf{Mix}         \\ 
        \midrule
        % Amazon                 & -           & 0.64459799  & 0.625786164 & 0.58528375  \\ \hline
        % DSLR                   & 0.535641603 & -           & 0.627358491 & 0.541855204 \\ \hline
        % Webcam                 & 0.549949949 & 0.646055276 & -           & 0.528092006 \\ \hline
        \textbf{Amazon}                 & -           & 0.28919598  & 0.251572328 & \textbf{0.1705675}    \\ 
        \rowcolor{table_gray}
        \textbf{DSLR}                   & 0.071283206 & -           & 0.254716982 & \textbf{0.083710408}  \\ 
        \textbf{Webcam}                 & 0.099899898 & 0.292110552 & -          & \textbf{0.056184012} \\
        \bottomrule
    \end{tabular}
}
\end{table}


% 探究 source 和 target 的相似性对实验结果的影响
 


\begin{figure*}[ht] % ht for here,top
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/exp03_similarity.pdf}
    \caption{An image of desk lamp from the original \textit{Webcam} and the ones from its perturbed versions. The main difference between the perturbed ones and the original is the brightness, contrast, Gaussian noise and motion blur.}
    \label{fig:exp03_similarity}
\end{figure*}

\textbf{Similarity}:  we then explore that how does the similarity between the source and target domains affect the usability of DAMIA. 


To this end, we create multiple similar datasets to obfuscate \textit{Webcam}. Instead of collecting similar samples, we generate similar samples by modifying original samples from \textit{Webcam} slightly. For example, the modification can be realized through the adjustment of the luminance and tools for that goal  \cite{hendrycks2019benchmarking} are available online \footnote{https://github.com/hendrycks/robustness}. Particularly,  brightness, contrast, Gaussian noise and motion blur are involved in our experiment to modify the original image as shown in  \autoref{fig:exp03_similarity}. Similar to the previous experiments, all the models are trained for 100 epochs, and membership inference attacks are deployed on those models. \autoref{tab:exp03_similarity} shows that accuracy of models are specifically enhanced with a excellent effectiveness achieved. 



%The results are shown in \autoref{tab:exp03_similarity}. It can be observed that the test accuracies on the target are also close to the ones on the source, which are nearly 100\% in these cases.  Moreover, the effectiveness of DAMIA is well kept.

% \red{Please note that in this case, the similarity between the similar source and the target is above 80\%, while in the case where the sources are \textit{Amazon} and \textit{DSLR}, the similarities are \textbf{0.593750} and \textbf{0.781250}.}  \ZY{These are irrelevant to our results. Better to include these in the table or caption. }
%Therefore, a similar dataset used to obfuscate the sensitive dataset in DAMIA has positive impact on both usability and effectiveness.







 

% \delete{ The idea is based on the observation that: in experiments of \textit{Q2}, no matter what adaptation direction is, either from \textit{DSLR} to \textit{Webcam} or \textit{Webcam} to \textit{DSLR}, test accuracy of the target domain is satisfactory. Visually, \textit{DSLR} and \textit{Webcam} are alike according \autoref{fig:office31}. } \ZY{There is no connection between that part and what you said here. How does it come into being? } \HW{This part is for explaining why we take similarity into consideration. So, seems unnecessary, I guess? Let's delete it.}



% \textbf{Similarity}: We further extend our exploration by raising the final question: will the high similarity between the source and target domains affect the effects of DAMIA, especially the test accuracy on the target? The question is posed based on the observation that: in \textit{Q2}, no matter what adaptation direction is (i.e. from \textit{DSLR} to \textit{Webcam} or \textit{Webcam} to \textit{DSLR}), test accuracy of the target domain is satisfactory, and visually, \textit{DSLR} and \textit{Webcam} are alike according \autoref{fig:office31}.
% We attempt to answer the question by performing experiments using source domains similar to the target domains. However, to craft a similar source domain to the target is not trivial. Instead of collect similar samples manually, we introduce perturbations to the samples from the target domain to obtain a similar one. That is, we introduce factors such as light condition to the samples of the target. \citet{hendrycks2019benchmarking} provides a method to produce images with specific perturbations. We use their tools\footnote{https://github.com/hendrycks/robustness} to build our similar source domains. Althought there are more than 15 perturbations that can be used for perturbation we choose 4 of them for our experiment, involving brightness, contrast, gaussian noise and motion blur. 
% We choose \textit{Webcam} as the target domain and create 4 similar source domains mentioned with the aforementioned perturbations. Their visual difference between the original one is shown in \autoref{fig:exp03_similarity}. The same as \textit{Q2}, we focus on the advantage of membership inference and the test accuracy on the target domain. Consistent with \textit{Q2}, all the models are trained for 100 epochs. 




\begin{table}[H]
    \centering
    \caption{Experiment results on similar source domains. The \textit{Original} stands for the \textit{Webcam} from Office-31. Please note that in this case, the similarity between the similar source and the target is above 0.8, while in the case where the sources are \textit{Amazon} and \textit{DSLR}, the similarities are \textbf{0.593750} and \textbf{0.781250}.}
    \label{tab:exp03_similarity}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    \tabincell{c}{\textbf{Adaptation} \\ \textbf{Direction}} & \tabincell{c}{ \textbf{Similarity} } & \tabincell{c}{\textbf{Train Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{Test Acc.}\\ \textbf{on Target}}  &  \tabincell{c}{\textbf{MIA Acc.}\\ \textbf{on Target}} & \tabincell{c}{\textbf{$adv_{mi}$}\\ \textbf{on Target}} \\ 
    \midrule
    \textbf{Brightness $\rightarrow$  Original   }  &  0.843750  & 0.993710692    & \textbf{1.0}         & \textbf{0.510220126} & \textbf{0.020440252}\\ 
    \rowcolor{table_gray}
    \textbf{Contrast $\rightarrow$  Original     }  &  0.843750  & 0.993710692    & \textbf{0.993710692} & \textbf{0.512578616} & \textbf{0.025157232}\\ 
    \textbf{Gaussian Noise $\rightarrow$ Original}  &  0.812500  & 0.988993711    & \textbf{0.974842767} & \textbf{0.522012579} & \textbf{0.044025158}\\ 
    \rowcolor{table_gray}
    \textbf{Motion Blur $\rightarrow$  Original  }  &  0.812500  & 0.995283019    & \textbf{0.993710692} & \textbf{0.512578616} & \textbf{0.025157232}\\ 
    \bottomrule
    \end{tabular}%
    } 
\end{table}

% Results are illustrated in \autoref{tab:exp03_similarity}.The experiments appears to be promising. It can be observed that the among 4 similar domains, the models with DAMIA using domains similar to the target demonstrate acceptable resistance to membership inference on the target domain. Moreover, the test accuracies on the target are also close to the ones on the source, which are nearly 100\% in these cases. Please note that in this case, the similarity between the similar source and the target is above 80\%, while in the case where the sources are \textit{Amazon} and \textit{DSLR}, the similarities are \textbf{0.593750} and \textbf{0.781250}. 
% Hence, by crafting a similar domain from the target domain with some perturbation and utilizing it as the source domain for DAMIA, a model with DAMIA enabled can not only lower the advantage of membership inference on the target but also push the test accuracy on the target as close to the ones on the source as possible. 

\ZY{Merge latex files of this Section into one not multiple ones. }


==> Trashbin/sec0-abstract.tex <==



==> Trashbin/sec7-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% \ZY{ I do not think the following discussions bring  more values to the paper. For the first part, why DAMIA works, we already explained it in our insight, and what you said here may confuse the reviewers. For the second part, these so-called limitations are not genuine limitations. Instead, you state two things there: (i) It seems that you implicitly admit that our method may hinder the usability.   (ii) you present the future works. For (i), you should never claim something like that. Our claim is we propose a novel method that counter MI attacks while maintaining the usability. Now you gives the reviewer excuses to kill the paper. For (ii), the future work should go to conclusion.  Anyway, it is up to you. If you want to keep them, you may want to polish them, and I will not argue against you if you can do that. }


% on the source domain, the advantage of membership inference does drop when the diversity of the source increase from 1 to 2. For example, the membership inference advantage are 0.28919598 and 0.251572328 when adapting from \textit{DSLR} or \textit{Webcam} to \textit{Amazon}. After mixing domains, the membership inference accuracy reduces to 0.1705675. Even though the source domain is not our focus, it might be of use when the privacy of the source domain is taken into consideration.

% \HW{maybe should place this part in disscussion? Or maybe I should just delete it.}
% 对于 source domain，有意料之外的效果, 在 source 上的 adv 下降了。
% 这里想表达的是，在实验的过程中，有一个无关文章核心的观察结果。就是说，尽管我们在实验上观察到 diversity 的变化对 DAMIA 的作用有限（无论是 effectiveness 还是 usability）。但是在实验中观察到，对于用来起混淆作用的 source domain，当我们将 diversity 提高之后，这种提高使得对 source domain 的成员推断攻击优势下降了（当然，我们之前只关注 target domain 上的成员推断攻击优势，因为是核心所在）。如果对 source domain 的隐私有所要求的话, DAMIA 也会有点作用，通过提高 diversity。可能也可以拓展其应用面。


% \red{However, we observe that in \autoref{tab:exp03_diversity_source_test_acc} for the source domain, the advantage of membership inference does drop when the diversity of the source increase from 1 to 2. For example, the membership inference advantage are 0.28919598 and 0.251572328 when adapting from \textit{DSLR} or \textit{Webcam} to \textit{Amazon}. After mixing domains, the membership inference accuracy reduces to 0.1705675. Even though the source domain is not our focus, it might be of use when the privacy of the source domain is taken into consideration.} \ZY{I am confused here. What do you mean? Can you explain it with Chinese? In our experiment, the dataset in source domain does not have another dataset involved that may obfuscate it, and its only functionality is to obfuscate the dataset in the target domain. Obviously, the source domain will not have any impact on its usability, so what are you argue for.  } \HW{try to claim the purpose of this part in Chinese. I put the claim in comments, please read it and see whether it helps for better understanding.}




% \begin{table}[H]
% \centering
% \caption{ Test accuracies on the source domains of different diversity. Please note that the diversity of Mix is 2.}
% \HW{will change the form of the table once this part is considered acceptable.}
% \label{tab:exp03_diversity_source_test_acc}
% \resizebox{0.48\textwidth}{!}{%
%     \begin{tabular}{ccccc}
%         \toprule
%         \diagbox{\textbf{Target}}{\textbf{$adv_{mi}$}}{\textbf{Source}} & \textbf{Amazon}      & \textbf{DSLR  }      & \textbf{Webcam}      & \textbf{Mix}         \\ 
%         \midrule
%         % Amazon                 & -           & 0.64459799  & 0.625786164 & 0.58528375  \\ \hline
%         % DSLR                   & 0.535641603 & -           & 0.627358491 & 0.541855204 \\ \hline
%         % Webcam                 & 0.549949949 & 0.646055276 & -           & 0.528092006 \\ \hline
%         \textbf{Amazon}                 & -           & 0.28919598  & 0.251572328 & \textbf{0.1705675}    \\ 
%         \rowcolor{table_gray}
%         \textbf{DSLR}                   & 0.071283206 & -           & 0.254716982 & \textbf{0.083710408}  \\ 
%         \textbf{Webcam}                 & 0.099899898 & 0.292110552 & -          & \textbf{0.056184012} \\
%         \bottomrule
%     \end{tabular}
% }
% \end{table}



% \subsection{Why DAMIA Works}

% Intuitively, DAMIA provides a way to obfuscate the sensitive dataset with an other related dataset, Since the original sensitive dataset is obfuscated, the membership inference fails. Theoretically, what is the principles underlying from a DL perspective? \red{ In this section, we give one possible explanation. In \autoref{sec:evaluation}, we observe that the model trained by DAMIA doesn't overfit or underfit on the training data from the dataset in the target domain.  
% Observed that among the experiment results in \autoref{sec:evaluation}, on the target domain, the  accuracy can be higher than the training accuracy with respect of the target domain in some cases, especially when the source domain has noticeable difference. For example, in the case of \texttt{MNIST} v.s. \texttt{SVHN}, test accuracies on target domain of both adoption direction(i.e. \texttt{MNIST} to \texttt{SVHN} and \texttt{SVHN} to \texttt{MNIST}) slightly exceed the training accuracies. Likewise, when domains are involved with \textit{Amazon} in \texttt{Office 31}, similar outcomes appear. Now that the model doesn't overfit the target domain, the success of membership inference descends\cite{yeom2018privacy}.}
% \ZY{I do not follow the logic of this section.}

% % imporve the DAMIA
% \subsection{Limitation of DAMIA}

% We admit that DAMIA also has some limitations  
% Since we are seeking to leverage domain adaption as a defense to membership inference on the target domain, we hope that the resulted models preserve high accuracy on the target with membership inference resistance. By using DAMIA, according to the experiments in \textbf{Q2} in \autoref{sec:evaluation}, a noticeable difference between the two domains has an impact on the test accuracy on the target domain. By crafting a dataset for source domain that is similar to the on in the target domain, we push the test accuracy upwards. 
% However, as a defense mechanism, DAMIA is far from delicate. We may automate the generation of the dataset for the source domain during training and automatically determine a suitable amount that will not burden the generation process heavily. Besides, we may design a better similarity metric so as to handle the case where tasks of DL models are image-irrelative. As for how to design a more practical defense mechanism to membership inference based on domain adaptation, we leave it as a future work.


\begin{table*} 
\centering
\caption{  Membership inference advantages on the source domains of different diversity. Please note that the diversity of Mix is 2.}
\label{tab:exp03_diversity_source_adv}
% \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{ccccccc}
        \toprule
        Sensitive Dataset & \multicolumn{6}{c}{Dataset for Obfuscation}                                     \\
        \cmidrule{2-7}
              & Amazon & DSLR & Webcam & Mix(Amazon $\oplus$ DSLR) & Mix(Amazon $\oplus$ Webcam) & Mix(DSLR $\oplus$ Webcam) \\ 
        \midrule
        Amazon            & -           & 0.28919598 & 0.251572328 & -                & -                  & \textbf{0.1705675} \\
        \rowcolor{table_gray}
        DSLR              & 0.071283206        & -           & 0.254716982 & -                & \textbf{0.083710408}      & -                   \\
        Webcam            & 0.099899898 & 0.292110552 & -           & \textbf{0.056184012}    & -                  & -                   \\
        \bottomrule
    \end{tabular}
    % }
\end{table*}

From experiments in \autoref{sec:evaluation}, we observe  that the on the target domain, models trained with DAMIA may have test accuracies slightly higher than training accuracies. It can be also attributed to the use of the source domain for obfuscation, which eventually prevent the model from overfitting the sensitive model, and may lead to underfitting. However, the difference between test accuracies and training accuracies is slight, it won't greatly harm the effective 

Besides, during the experiments to explore the effect of diversity, although we find that the diversity has limited contribution on the target domain; however, we notice a different outcomes on the source domain. In \autoref{tab:exp03_diversity_source_adv}, we can observe that the advantage of membership inference does drop when the diversity of the source increase from 1 to 2. For example, the membership inference advantage are 0.28919598 and 0.251572328 when adapting from \textit{DSLR} or \textit{Webcam} to \textit{Amazon}. When using a source domains with the diversity of 2, the membership inference accuracy reduces to 0.1705675. Therefore, DAMIA may be of use when the privacy of the source domain is taken into consideration.
